Restricted Strong Convexity of Deep Learning Models with Smooth Activations

We consider the problem of optimization of deep learning models with smooth activation functions. While there exist influential results on the problem from the ``near initialization'' perspective, we shed considerable new light on the problem. In particular, we make two key technical contributions for such models with $L$ layers, $m$ width, and $\sigma_0^2$ initialization variance. First, for suitable $\sigma_0^2$, we establish a $O(\frac{\text{poly}(L)}{\sqrt{m}})$ upper bound on the spectral norm of the Hessian of such models, considerably sharpening prior results. Second, we introduce a new analysis of optimization based on Restricted Strong Convexity (RSC) which holds as long as the squared norm of the average gradient of predictors is $\Omega(\frac{\text{poly}(L)}{\sqrt{m}})$ for the square loss. We also present results for more general losses. The RSC based analysis does not need the ``near initialization" perspective and guarantees geometric convergence for gradient descent (GD). To the best of our knowledge, ours is the first result on establishing geometric convergence of GD based on RSC for deep learning models, thus becoming an alternative sufficient condition for convergence that does not depend on the widely-used Neural Tangent Kernel (NTK). We share preliminary experimental results supporting our theoretical advances.

==> arXiv_RSC/app/arx1app_ntk.tex <==


\theontk*

\proof Let $\alpha^{(L+1)} = \frac{1}{\sqrt{m_L}} \v^\top \alpha^{(L)}$ be the output for any single input $x$, and let $A^{(L+1)} = [\alpha^{(L+1)}_i] \in \R^n$ be the vector of outputs for the dataset $\{x_i, i \in [n]\}$. The corresponding Jacobian is
\begin{align*}
J = \left[ \frac{\partial A^{(L+1)}}{\partial \vec(W^{(1)})}~,\ldots, ~\frac{\partial A^{(L+1)}}{\partial \vec(W^{(L)})}~, \frac{\partial A^{(L+1)}}{\partial \v} \right] \in \R^{n \times \sum_{l=1}^L m_{l-1} m_l + m_{L+1}}~,
\end{align*}
where $m_0 =d$ and $m_l =m$ for $l=1,\ldots,L+1$. Then, the kernel at initialization is
\begin{align*}
K_{\ntk}(\cdot ;\theta_0) = J J^\top &= \sum_{l=1}^L  \left[ \frac{\partial A^{(L+1)}}{\partial \vec(W^{(1)})}\right] \left[ \frac{\partial A^{(L+1)}}{\partial \vec(W^{(l)})}\right]^\top + \left[\frac{\partial A^{(L+1)}}{\partial \v} \right] \left[ \frac{\partial A^{(L+1)}}{\partial \v}\right]^\top~.
\end{align*}
Note that
\begin{align*}
\left[\frac{\partial A^{(L+1)}}{\partial \v}\right] \left[  \frac{\partial A^{(L+1)}}{\partial \v}\right]^\top =  \frac{1}{m_L}A^{(L)} (A^{(L)})^\top~.
\end{align*}
Recall that by chain rule, for any $l \in [L]$
\begin{align*}
\frac{\partial \alpha^{(L+1)}}{\partial \vec(W^{(l)})} & = \frac{\partial \alpha^{(l)}}{\partial \vec(W^{(l)})} \frac{\partial \alpha^{(L+1)}}{\partial \alpha^{(l)}}  
 = \frac{\partial \alpha^{(l)}}{\partial \vec(W^{(l)})}  \left( \prod_{l'=l+1}^L \frac{\partial \alpha^{(l')}}{\partial \alpha^{(l'-1)}} \right) \frac{\partial \alpha^{(L+1)}}{\partial \alpha^{(L)}} \\
& = \frac{1}{\sqrt{m_{l-1}}} \alpha^{(l-1)} D_l \left( \prod_{l'=l+1}^L \frac{1}{\sqrt{m_{l'-1}}}  W^{(l')} D_{l'} \right) \frac{1}{\sqrt{m_L}} \v ~. 
\end{align*}
where $D_l = [\text{diag}(\phi'(\tilde{\alpha}^{(l)}))] \in \R^{m_l \times m_l}$ are diagonal matrices with elements which are gradients of the activation. Then, in matrix notation
\begin{align*}
\left[ \frac{\partial A^{(L+1)}}{\partial \vec(W^{(l)})} \right] \left[ \frac{\partial A^{(L+1)}}{\partial \vec(W^{(l)})} \right]^\top = \frac{1}{m_{l-1}} A^{(l-1)} (A^{(l-1)})^\top \odot B_l B_l^\top 
\end{align*}
where for $l \in [L]$
\begin{align}
B_l & =  D_l \left( \prod_{l'=l+1}^L \frac{1}{\sqrt{m_{l'-1}}}  W^{(l')} D_{l'} \right) \frac{1}{\sqrt{m_L}} \v ~.
\end{align}
In particular, note that
\begin{align*}
    B_L = \frac{1}{\sqrt{m_{L}}} D_L  \v~,\qquad \text{and} \qquad B_{L-1} = \frac{1}{\sqrt{m_{L-1} m_{L}}} D_{L-1} W^{(L)} D_L \v~. 
\end{align*}
As a result, 
\begin{align*}
JJ^\top & = \sum_{l=1}^L \frac{1}{m_{l-1}} A^{(l-1)} (A^{(l-1)})^\top \odot B_l B_l^\top + \frac{1}{m_L} A^{(L)} (A^{(L)})^\top~.
\end{align*}
From the Schur product theorem~ (e.g., see~\cite[Lemma 6.5]{oymak2020hermite},\cite[Theorem~3.2]{QN-PB-MM:21}), for positive semi-definite matrices (PSD) $P,Q \in \R^{n \times n}$, it holds that $\lambda_{\min}(P \odot Q) \geq \lambda_{\min}(P) \min_{i \in [n]} Q_{ii}$. Then,
\begin{align}
\lambda_{\min}(JJ^\top) \geq \sum_{l=1}^L \frac{1}{m_{l-1}} \lambda_{\min}\left(A^{(l-1)} (A^{(l-1)})^\top\right)  \min_{i \in [n]} \| (B_l)_{i,:}\|_2^2 + \frac{1}{m_L} \lambda_{\min}\left(A^{(L)} (A^{(L)})^\top\right)~.
\end{align}
Then, for any $l \in [L]$, we want to lower bound $\lambda_{\min}\left(A^{(l)} (A^{(l)})^\top\right)$ and  $\min_{i \in [n]} \| (B_l)_{i:}\|_2^2$. In fact, it suffices to lower bound $\lambda_{\min}\left(A^{(L)} (A^{(L)})^\top\right)$. Following Theorem~\ref{theo:mineig} (Section~\ref{sec:arXiv_ntk}), for $m_l = m, l \in [L]$, with probability at least $1-\delta - \frac{4L}{m}$, we have $\lambda_{\min}\left(A^{(L)} (A^{(L)})^\top\right) \geq c_0 m_L \lambda_1$, where $c_0 = \max_{r > 1} c_0^{(L-1,r)}$ and $c_0^{(l,r)}$ is as in Theorem~\ref{theo:mineig}. \pccomment{How to know that $c_0$ is well defined? We would need to ensure that $c_0:=\max_{r > 1} c_0^{(L-1,r)}$ is bounded and that the maximum is actually attained. Looking at Theorem~\ref{theo:mineig} it seems that we need $\sigma_0^2\leq 2$, otherwise the quantity $c_0$ seems to be unbounded. Are we ensuring this?} \abcomment{This is a lower bound, so large $c_0$ is not a worry. Also, the Hermite coefficients decrease quickly as $r$ increases, so larger values of $r$ will lead to smaller $c_0^{l,r}$. I had derived these terms exactly for GeLU activations, its in the appendix of the old version, maybe will bring that here.}\pccomment{I see. As I understood, you might include the GeLU case in the Appendix.} Plugging this back,
\begin{align*}
\lambda_{\min}(K_{ntk}(\cdot ;\theta_0)) = \lambda_{\min}(JJ^\top)\geq \frac{1}{m_L} \lambda_{\min}\left(A^{(L)} (A^{(L)})^\top\right) \geq c_0 \lambda_1~,
\end{align*}
with probability at least $1-\delta - \frac{4L}{m}$. This completes the proof. \qed 

\mineig*

\proof There are three key parts to the proof: 
\begin{enumerate}[(a)]
\item  showing that under suitable conditions, the minimum eigenvalue of $A^{(l)} (A^{(l)})^\top$ for a model with width $\tilde{\Omega}(n)$ can be lower bounded by a constant scaled version of the minimum eigenvalue of the expectation $\E[A^{(l)} (A^{(l)})^\top]$, i.e., a matrix concentration bound; 
\item establishing suitable upper and lower bounds for $\| \alpha^{(l)}\|_2^2$, in particular $\| \alpha^{(l)}\|_2^2 = \Theta(m_l)$ with high probability, which satisfies conditions needed for the matrix concentration result in (a) above and also helps lower bounding the minimum eigenvalue of the expectation $\E[A^{(l)} (A^{(l)})^\top]$ in (c) below; and 
\item lower bounding the minimum eigenvalue of the expectation $\E[A^{(l)} (A^{(l)})^\top]$ using generalized Hermite series expansion to handle multiple layers of inhomogenous activations and lower bounds on $\| \alpha^{(l)}\|_2^2$ as in (b) above.
\end{enumerate}
Next we get into the details of each of these results.

\noindent {\bf (a) Matrix Concentration.} Note that by construction $A^{(l)} = \phi( \frac{1}{\sqrt{m_{l-1}}} A^{(l-1)} (W_0^{(l)})^\top) \in \R^{n \times m_l}$, where $W_0^{(l)} \in \R^{m_{l} \times m_{l-1}}$ and $w_{0,ij}^{(l)} \sim \cN(0,\sigma^2)$. In our setting $\sigma^2 = \nu_0^2 = \frac{\sigma_0^2}{c_{\phi,\sigma_0}}$. Then, 
\begin{align}
\E_{W_0^{(l)}}[A^{(l)} (A^{(l)})^\top] = m_l \E_{g \sim 
\cN(\bm{0}_{m_{l-1}},\sigma^2 \I_{m_{l-1}})
}\left[ \phi \left( \frac{1}{\sqrt{m_{l-1}}} A^{(l-1)} g \right) \phi\left( \frac{1}{\sqrt{m_{l-1}}} A^{(l-1)} g) \right)^\top \right]~.
\end{align}
The minimum eigenvalue of the right hand side above can lead to a high probability bound of the random matrix $A^{l} (A^{l})^\top$ as shown in the following Lemma~\ref{lemm:highproblambda}. The proof is in Section~\ref{ssec:highprobablambda}.

\highproblambda*

% \begin{restatable}[{\bf Matrix Concentration}]{lemm}{highproblambda}
% Let
% \begin{align}
% \lambda_l := \lambda_{\min}\left(  \E_{g \sim \sigma^2 \I_{m_{l-1}}}\left[ \phi \left( \frac{1}{\sqrt{m_{l-1}}} A^{(l-1)} g \right) \phi \left( \frac{1}{\sqrt{m_{l-1}}} A^{(l-1)} g \right)^\top \right] \right) ~,
% \end{align}
% and
% \begin{align}
% m_{l} \geq \max \bigg( n, c_2 v \max\big(1, \log(15 v)\big) \log (Ln/\delta) \bigg) ~ ,
% \end{align}
% where $v := \frac{2(\sqrt{\log n}+1)^2 \sigma^2 \| A^{(l-1)}\|_F^2}{c_3 \lambda_l m_{l-1}}$, and $c_2, c_3$ are absolute constants. Then, with probability at least $(1-\frac{\delta}{L})$ over the draw of $W^{(l)}_0$, we have 
% \begin{align}
% \lambda_{\min}( A^{(l)} (A^{(l)})^\top ) \geq \frac{m_{l} \lambda_l}{4}~.
% \end{align}
% \label{lemm:highproblambda}
% \end{restatable}
Then, it suffices to upper bound $\| A^{(l-1)} \|_F^2$ and lower bound $\lambda_l$ for $\sigma^2 = \nu_0^2 = \frac{\sigma_0^2}{c_{\phi,\sigma_0}}$.


\noindent {\bf (b) Bounding $\|A^{(l)}\|_F^2$.} To bound the Frobenius norm $\| A^{(l)} \|_F^2$, we focus on bounding the $L_2$ norm of each row of $A^{(l)}$ and show that $\|\alpha^{(l)}(x)\|_2^2 = \Theta(m_l)$. In Lemma~\ref{lemm:alphainit1} below, we show that the bound holds uniformly over the dataset $\{x_i, i\in [n]\}$ with high probability. The proof is in Section~\ref{ssec:alphainit}.
\alphainit*

% \begin{restatable}[{\bf Bounding $\| \alpha^{(l)}(x)\|_2^2$}]{lemm}{alphainit}
% Let $\{\alpha^{(l)}(x_i) \in \R^{m_l}, i \in [n]\}$ be the set of output at layer $l$ at initialization for the set of inputs $\{ x_i, i \in [n]\}$. Let $c_{\phi, \sigma_0} := \E_{z \sim \cN(0,\sigma_0^2)}[\phi^2(z)]$, $\nu_0^2 := \frac{\sigma_0^2}{c_{\phi,\sigma_0}}$, and $h_C(l) := \sum_{i=0}^l \nu_0^{2i}$. Let the depth $L$ be such that $\max\left(\frac{8h_c^2(L)}{c_{\phi,\sigma_0}^2} , \frac{4 h_c(L)}{c_{\phi,\sigma_0}} \right) \leq \sqrt{m}$. Assuming the elements of $W_0^{(l)}, l \in [L]$ are drawn i.i.d.~from $\cN(0,\nu_0^2)$, with probability at least $1 - \frac{2L}{m^2}$ over the draw of $\{W^{l'}_0, l'\in [L] \}$, uniformly over $l \in [L]$ and $i \in [n]$, we have 
% \begin{align*}
% \frac{c_{\phi,\sigma_0}}{2} m_l \leq c_{\phi,\sigma_0}\left(1 -  \frac{h_C(l)}{2h_C(L)}\right) m_l  \leq  \| \alpha^{(l)}(x_i) \|_2^2  \leq c_{\phi,\sigma_0} \left(1 + \frac{h_C(l)}{2h_C(L)}\right) m_l \leq \frac{3 c_{\phi,\sigma_0}}{2} m_l~.
% \end{align*}
% \label{lemm:alphainit1}
% \end{restatable}
As a result, by union bound, with probability at least $(1 - 2n\sum_{l=1}^L\frac{1}{m_l^2}) \geq (1 - 2\sum_{l=1}^L\frac{1}{m_l}))$ for $m_l \geq n$,
%
%$(1 - \frac{2nL}{m^2}) \geq (1 - \frac{2L}{m})$ for $m \geq n$,
%
uniformly over $l \in [L]$, we have 
\begin{align}
\| A^{(l)} \|_F^2 = \sum_{i=1}^n \| \alpha^{(l)}(\x_i)\|_2^2 \leq \frac{3 c_{\phi,\sigma_0}}{2}n m_{l} ~.
\label{eq:frobupper0}
\end{align}
%\abcomment{for simplicity, assuming $\phi(0) =0$, satisfied by almost all activation functions folks use}
Then, since $\nu_0^2 = \frac{\sigma_0^2}{c_{\phi,\sigma_0}}$, in Lemma~\ref{lemm:highproblambda}, we have $v \leq c_2 \frac{\sigma_0^2 n \log n}{\lambda_l}$, for some constant $c_2>0$. 
%\abcomment{the term \pc{$\frac{m_l}{m_{l-1}}$} was added here which does not look correct, since Lemma 6.1 depends on $\| A^{(l-1)}\|_F^2$, so the $m_{l-1}$ cancels out.}
%%\pccomment{This bound holds if $\log n\geq 1$, which makes sense since typically $n\geq 3$; I guess we shouldn't care much about this.} 
For $L =O(1)$, $h_C^4(L) = O(1) \leq m_l$. As a result, for $l \in [L]$, it suffices to have
%\abdelete{\pc{\begin{align*}
%m_{l} & \geq \max\left( n ~,~ c_2 \frac{\sigma_0^2 n \log n}{\lambda_l}\frac{m_l}{m_{l-1}} \max\left(1, \log \left( c_3 \frac{\sigma_0^2 n \log n}{\lambda_l}\frac{m_l}{m_{l-1}} \right) \right) \log \frac{Ln}{\delta}  \right) \overset{(a)}{=} \tilde{\Omega}(n)~,
%\end{align*}
%and so under the assumption that $m_l=m$, $l\in[L]$,}}
\begin{align}
m_{l} & \geq \max\left( n ~,~ c_2 \frac{\sigma_0^2 n \log n}{\lambda_l} \max\left(1, \log \left( c_3 \frac{\sigma_0^2 n \log n}{\lambda_l} \right) \right) \log \frac{Ln}{\delta}  \right) \overset{(a)}{=} \tilde{\Omega}(n)~,
\end{align}
where (a) holds as long as $\lambda_l = \Omega(1)$, which holds with high probability as we show next.
%Thus, in terms of the dependence on the sample size $n$, $m = \tilde{\Omega}(n)$ suffices.

%\abedit{... this should follow by standard analysis, including our results in Section 3, and Lemma C.1 in [NMM21], although we want to (and should be able to) drop the $-\exp(-\Omega(d))$ term in the 'bad probability' part of their result.}

\noindent {\bf (c) Lower Bounding $\lambda_l$.} Next, we focus on lower bounding $\lambda_l$, which  Following  Lemma~\ref{lemm:hermprod}, $\lambda$ can be lower bounded by the minimum eigenvalue of the inner product of matrices  ${A^{(l-1)}}^{\star r}$, whose rows are the row-wise Kronecker products of the rows of $A^{(l-1)}$~\cite{oymak2020hermite,ng2021hermite2}. The result is stated in Lemma~\ref{lemm:lambdahermite} and the proof is in Section~\ref{ssec:lambdahermite}.

%\abcomment{result below needs a bit of work}

\lambdahermite*

% \begin{restatable}{lemm}{lambdahermite}
% Let $c_{\phi,\sigma_0} := \E_{z \sim cN(0,\sigma_0^2}[\phi^2(z)]$, and $\nu_0 := \frac{\sigma_0^2}{c_{\phi,\sigma_0}}$. Let $\mu_r^{[q]}(\phi), q>0$ be the $r$-th generalized Hermite coefficient corresponding to the generalized Hermite series expansion w.r.t.~$H_r^{[q]}$ of $\phi$. Let $c_{l,i} = \frac{\| \alpha^{(l)}(x_i) \|_2}{\sqrt{m_l}}$ and $(\mu_{r,0}^{(l)})^2 = \min_{i \in [n]} \left( \mu_r^{[c_{l,i}^2 \sigma^2]} (\phi) \right)^2$. For any integer $r > 0$,  with probability at least $1-\frac{4L}{m}$, uniformly over $l \in [L]$ we have
% \begin{align*}
% \lambda_{\min}\left(  \E_{g \sim \sigma^2 \I_{m_{l}}}\left[ \phi\left( \frac{1}{\sqrt{m_{l}}} A^{(l)} g \right) \phi\left( \frac{1}{\sqrt{m_{l}}} (A^{(l)} g)^\top\right) \right] \right) 
% %& \geq \left( \mu_r^{[\nu_0^2]}(\phi) \right)^2 \frac{\nu_0^{6r}c_{l}^{2r}}{m_{l}^r} \lambda_{\min}( {A^{(l)}}^{\star r} ({A^{(l)}}^{\star r})^\top  ) \\
%  & \geq \left( \frac{(\mu_{r,0}^{(l)})^2}{6 c_{\phi,\sigma_0}} \right)^l \left( \frac{\sigma_0^2}{2} \right)^{3rl} \lambda_{1} 
% % & (\mu_{r,0}^{(l)})^2 \left( \frac{\sigma_0^2}{2} \right)^{3r} \left( \frac{\sigma_0^2}{c_{\phi,\sigma_0}} \right)^{3rl} \left( \frac{\mu_r^{[\sigma^2]}(\phi)}{2} \right)^{2l} \lambda_{\min}(XX^\top)~.
% \end{align*}
% %where $\bar{A}_{l}_{(i,:)} = \| A_{l}_{(i,:)} \|_2 A_{l}_{(i,:)}$. \abcomment{the $\bar{A}$ bit can be simplified based on lower bounds on the row norms}
% \label{lemm:lambdahermite}
% \end{restatable}
Let $c_0^{(l,r)} = \left( \frac{(\mu_{r,0}^{(l)})^2}{6 c_{\phi,\sigma_0}} \right)^l \left( \frac{\sigma_0^2}{2} \right)^{3rl}$. Then, combining Lemma~\ref{lemm:highproblambda} and Lemma~\ref{lemm:lambdahermite}, with probability at least $1-\delta - \frac{4L}{m}$, we have 
\begin{align*}
\lambda_{\min}(A^{(l)} (A^{(l)})^\top ) \geq \frac{m_l}{4} \lambda_l \geq c_0^{(l-1,r)} m_l \lambda_1~.
\end{align*}
That completes the proof. \qed 





\subsection{Proof of Lemma~\ref{lemm:highproblambda}}
\label{ssec:highprobablambda}
We start with a variant of Lemma~\ref{lemm:outl2} which explicitly shows that the output $\| \alpha^{(l)}\|_2$ is sub-Gaussian for Gaussian random weights. For simplicity, we assume $\phi(0)=0$, noting that the result can be extended to the general case straightforwardly.

\begin{lemm}
Let $A^{(l)} = [ \alpha^{(l)}(x_i)] \in \R^{n \times m_l}$ be the outputs of layer $l$.
For $g \sim \cN(\bm{0}_{m_{l-1}},\sigma^2 \I_{m_{l-1}})$, let $\vartheta^{(l)} = \phi(\frac{1}{\sqrt{m_{l-1}}} A^{(l-1)} g ) \in \R^{n}$. Then, $\| \vartheta^{(l)}\|_2$ is a sub-Gaussian random variable with 
\begin{align*}
\| \|\vartheta^{(l)}\|_2 \|_{\psi_2} = \left\| \left\| \phi\left(\frac{1}{\sqrt{m_{l-1}}} A^{(l-1)} g \right) \right\|_2 \right\|_{\psi_2} \leq c \frac{\sqrt{2} (\sqrt{\log n} + 1)\sigma}{\sqrt{m_{l-1}}} \| A^{(l-1)} \|_F
\end{align*}
for some absolute constant $c>0$.
\label{lemm:gammasubg}
\end{lemm}
\proof First, note that since $\phi$ is 1-Lipschitz and $\phi(0) = 0$, we have $\norm{\phi( \frac{1}{\sqrt{m_{l-1}}} A^{(l-1)} g )}_2 \leq \norm{\frac{1}{\sqrt{m_{l-1}}} A^{(l-1)} g}_2$. Now, 
\begin{align*}
\P  \left( \left\| \frac{1}{\sqrt{m_{l-1}}} A^{(l-1)} g \right\|_2^2 \geq \epsilon^2 \frac{1}{m_{l-1}} \| A^{(l-1)} \|_F^2 \right)
& = \P \left( \frac{1}{m_{l-1}} \sum_{i=1}^n \langle \alpha_i^{(l-1)}, g \rangle^2 \geq \epsilon^2 \frac{1}{m_{l-1}} \sum_{i=1}^n \| \alpha_i^{(l-1)} \|_2^2 \right)\\
& \leq \sum_{i=1}^n \P \left( \frac{1}{m_{l-1}} \langle \alpha_i^{(l-1)}, g \rangle^2 \geq \epsilon^2 \frac{1}{m_{l-1}} \| \alpha_i^{(l-1)} \|_2^2 \right) \\
& = \sum_{i=1}^n \P \left( |\langle \alpha_i^{(l-1)}, g \rangle| \geq \epsilon \| \alpha_i^{(l-1)} \|_2 \right)\\
& \leq 2n \exp\left( - \frac{\epsilon^2}{2\sigma^2} \right)~.
\end{align*}
In other words, with $\tilde{\epsilon} = \frac{\epsilon}{\sqrt{m_{l-1}}} \| A^{(l-1)} \|_F$, for all $\tilde{\epsilon} > 0$ we have 
\begin{align*}
\P \left( \left\| \frac{1}{\sqrt{m_{l-1}}} A^{(l-1)} g \right\|_2 \geq \tilde{\epsilon} \right) \leq 2n \exp\left( - \frac{m_{l-1} \tilde{\epsilon}^2}{2\sigma^2 \| A^{(l-1)} \|^2_F } \right) ~.
\end{align*}
Now, with $\tilde{\epsilon} = \frac{\sigma \sqrt{2 \log n} }{\sqrt{m_{l-1}}} \| A^{(l-1)} \|_F + \epsilon $, for all $\epsilon > 0$ we have
\begin{align*}
\P \left( \left\| \frac{1}{\sqrt{m_{l-1}}} A^{(l-1)} g \right\|_2  \geq  \frac{\sigma \sqrt{2 \log n}}{\sqrt{m_{l-1}}} \| A^{(l-1)} \|_F + \epsilon  \right) & \leq 2n \exp \left( - \log n \right)  \exp\left( - \frac{m_{l-1} \epsilon^2}{2\sigma^2 \| A^{(l-1)} \|^2_F } \right) \\
\Rightarrow ~~~\P \left( \left\| \phi\left( \frac{1}{\sqrt{m_{l-1}}} A^{(l-1)} g \right) \right\|_2  \geq  \frac{\sigma \sqrt{2 \log n }}{\sqrt{m_{l-1}}} \| A^{(l-1)} \|_F + \epsilon  \right) & \leq 2 \exp\left( - \frac{m_{l-1} \epsilon^2}{2\sigma^2 \| A^{(l-1)} \|^2_F } \right)~.
\end{align*}
Then, from Proposition~\ref{prop:subgsum}, it follows that $\| \phi( \frac{1}{\sqrt{m_{l-1}}} A^{(l-1)} g ) \|_2$ is sub-Gaussian with 
\begin{align*}
\left\| \left\| \phi\left( \frac{1}{\sqrt{m_{l-1}}} A^{(l-1)} g \right) \right\|_2 \right\|_{\psi_2} \leq c \frac{\sqrt{2} (\sqrt{\log n} + 1)\sigma}{\sqrt{m_{l-1}}} \| A^{(l-1)} \|_F~,
\end{align*}
for some absolute constant $c$. This completes the proof. \qed 

\begin{prop}
Let $a_1, a_2 > 0$. If a non-negative random variable $Z$ satisfies $\P( Z \geq a_1 + \epsilon) \leq 2 \exp(-\epsilon^2/a_2^2)$, then $\| Z \|_{\psi_2} \leq c(a_1 + a_2)$, where $c$ is an absolute constant.
\label{prop:subgsum}
\end{prop}
\proof Note that $Z-a_1 = [Z-a_1]_- + [Z-a_1]_+$. Since $Z$ is non-negative, $|[Z-a_1]_-| \leq a_1$ implying $\|[Z-a_1]_-\|_{\psi_2} \leq c_1 a_1$, where $c_1$ is an absolute constant. Further, by definition, $[Z-a_1]_+$ is sub-Gaussian with $\| [Z-a_1]_+ \|_{\psi_2} \leq c_2 a_2$, where $c_2$ is an absolute constant. Now, by triangle inequality
\begin{align*}
\| Z \|_{\psi_2} & = \| a_1 + [Z-a_1]_- + [Z - a_1]_+ \|_{\psi_2} \\
& \leq a_1 + \|[Z-a_1]_-\|_{\psi_2} + \| [Z-a_1]_+ \|_{\psi_2} \leq a_1 + c_1 a_1 + c_2 a_2\\
& \leq c(a_1+a_2)~,
\end{align*}
where $c = \max(1+c_1, c_2)$. That competes the proof. \qed

% \abcomment{update the analysis -- can be done more directly, using Hoeffding(?)} Let $U = \left\{u_i = \frac{\alpha_i}{\| \alpha_i\|_2}, i \in [n]\right\}$ so that $u_i \in \R^{m_l}, i \in [n]$. Then, from Lemma~\ref{lem:newaux1}, with probability at least $(1-2\exp(-\tau^2/(2\sigma_0^2)))$, we have 
% \begin{align*}
% \frac{1}{\| \alpha_i^{(l-1)} \|_2} \| W_0^{(l)} \alpha_i^{(l)} \|_2  =  \| W_0^{(l)} u_i \|_2 \leq \sigma_0(\sqrt{m} + \sqrt{\log n}) + \tau~,
% \end{align*}
% since $W_0^{(l)} \in \R^{m_{l} \times m_{l-1}}$ has entries $w_{0,ij}^{(l)} \sim \cN(0,\sigma_0^2)$.
% % Then, from the proof on Lemma~\ref{lemm:outl2} and Assumption~\ref{asmp:ginit}, with probability at least $(1-2\exp(-\tau^2/(2\sigma_0^2)))$, we have 
% % \begin{align*}
% % ~\frac{1}{\| \alpha_i^{(l-1)} \|_2} \| W^{(l)} \alpha_i^{(l-1)} \|_2  \leq \sqrt{m}\left( \sigma_1 + \frac{\rho}{\sqrt{m}} \right) + \tau = \sqrt{m} \gamma + \tau~.
% % \end{align*}
% Since $\phi(0)=0$, with probability at least $(1-2\exp(-\tau^2/(2\sigma_0^2)))$, we have 
% \begin{align*}
% \| \alpha_i^{(l)} \|_2 & \leq ~\left\| \frac{1}{\sqrt{m_{l-1}}} W_0^{l} \alpha_i^{(l-1)} \right\|_2 
%  \leq \left(\gamma + \frac{\tau  }{\sqrt{m}} \right) \| \alpha_i^{(l-1)} \|_2~.
% \end{align*}
% Then, with probability at least $(1-2\exp(-\tau^2/(2\sigma_0^2)))$, we have 
% \begin{align*}
% \| \Gamma^{(l)} \|^2_2 & = \sum_{i=1}^n \left\| \phi\left( \frac{1}{\sqrt{m}} \langle \alpha_i^{(l-1)}, g \rangle\right) \right\|^2_2 \leq  \left(\gamma + \frac{\tau  }{\sqrt{m}} \right)^2 \| A^{(l-1)} \|_F^2~\\
% \Rightarrow \qquad \| \Gamma^{(l)} \|_F & \leq \gamma \| A^{(l-1)} \|_F + \frac{ \tau \| A^{(l-1)} \|_F}{\sqrt{m}}~.
% \end{align*}
% Then, with $t = \frac{ \| A^{(l-1)} \|_F}{\sqrt{m}} \tau$, we have with probability at least $(1 - 2\exp(-\frac{m t^2}{2 \sigma_0^2 \| A^{(l-1)} \|_F^2})$, we have 
% \begin{align*}
% \| \Gamma^{(l)} \|_F \leq \gamma \| A^{(l-1)} \|_F + t~,
% \end{align*}
% Then, from \abedit{Proposition ??} it follows that $\| \Gamma^{(l)} \|_F$ is a sub-Gaussian random variable with $\| \Gamma^{(l)} \|_{\psi_2} \leq \gamma \| A^{(l-1)}\|_F + \frac{\sigma_0 \| A^{(l-1)} |_F}{\sqrt{m}} \leq \left( \gamma + \frac{\sigma_1}{\sqrt{m}} \right) \| A^{(l-1)}\|_F$, since $\sigma_0 \leq \sigma_1$. That completes the proof. \qed 

We are now ready to prove Lemma~\ref{lemm:highproblambda}.

\highproblambda*

\proof Recall that  $A^{(l)} = \phi( \frac{1}{\sqrt{m_{l-1}}} A^{(l-1)} (W_0^{(l)})^\top) \in \R^{n \times m_l}$, where $W_0^{(l)} \in \R^{m_{l} \times m_{l-1}}$ and $w_{0,ij}^{(l)} \sim \cN(0,\sigma^2)$, and that $\vartheta^{(l)} = \phi(\frac{1}{\sqrt{m_{l-1}}} A^{(l-1)} g) \in \R^{n}$. If $m_l < n$, then $\lambda_{\min}(A^{(l)} (A^{(l)})^\top) = 0$. So, we assume $m_l \geq n$.
%
Let $w_j \in \R^{m_{l-1}}$ denote the $j$-th row of $W_0^{(l)}$.
Let $\hat{A}^{(l)} \in \R^{n \times m_l}$ so that $\hat{A}_{:,j}^{(l)} = \phi( \frac{1}{\sqrt{m_l}} A^{(l-1)} w_j^\top ) \1_{[\| \phi(\frac{1}{\sqrt{m_l}} A^{(l-1)} w_j^\top \|_2 \leq t]}$ and $\hat{\vartheta}^{(l)} = \phi( \frac{1}{\sqrt{m_l}} A^{(l-1)} g ) \1_{[\| \phi(\frac{1}{\sqrt{m_l}} A^{(l-1)} g \|_2 \leq t]} \in \R^n$. Then, we have 
%\lzcomment{I did not find the proof of $\lambda_{\max}$?}
\begin{align*}
(i)\;\; &
\lambda_{\min}( A^{(l)} ( A^{(l)})^\top ) \geq \lambda_{\min}( \hat{A}^{(l)} ( \hat{A}^{(l)})^\top )  ~,\\
(ii)\;\;&\lambda_{\max}( \hat{A}_{:,j}^{(l)} ( \hat{A}_{:,j}^{(l)})^\top ) \leq t^2~,
\end{align*}
where (i) follows immediately by definition of $\hat{A}^{(l)}$ and (ii) follows since for any unit vector $v \in \R^n$, 
%\begin{align*}
$v^\top \hat{A}_{:,j}^{(l)} ( \hat{A}_{:,j}^{(l)})^\top v = \langle v, \hat{A}_{:,j}^{(l)} \rangle^2 \leq \| \hat{A}_{:,j}^{(l)} \|_2^2 \leq t^2$.
%\end{align*}

From Lemma~\ref{lemm:gammasubg}, we know that $\| \| \vartheta^{(l)} \|_2 \|_{\psi_2} \leq c_1  \frac{\sqrt{2}(\sqrt{\log n}+1)\sigma}{\sqrt{m}} \| A^{(l-1)} \|_F$.  Recall that for any subGaussian random variable $Z$, $\P(Z \geq t) \leq \exp(1-c t^2/\| Z \|_{\psi_2}^2)$ for some absolute constant $c$. For our analysis with $\| \vartheta^{(l)} \|_2$, for a suitable constant $a > 0$ we will use 
\begin{align}
    t = \frac{  \sqrt{2} (\sqrt{\log n}+1) \sigma \| A^{(l-1)} \|_F}{\sqrt{cm_{l-1}}} \sqrt{ \max \left(1 , \log \frac{2a (\sqrt{\log n} + 1)^2 \sigma^2 \| A^{(l-1)} \|_F^2}{ c \lambda_l m_{l-1}} \right) }~.
\label{eq:thres}
\end{align}

Let
\begin{align*}
\hspace*{-10mm}
G & := \E_{g \sim \cN(\bm{0}_{m_{l-1}},\sigma^2 \I_{m_{l-1}})}\left[ \vartheta^{(l)} (\vartheta^{(l)})^\top \right] = \E_{g \sim \cN(\bm{0}_{m_{l-1}},\sigma^2 \I_{m_{l-1}})}\left[ \phi\left( \frac{1}{\sqrt{m_{l-1}}} A^{(l-1)} g \right) \phi\left( \frac{1}{\sqrt{m_{l-1}}} A^{(l-1)} g \right)^\top \right] ~, \\
\hat{G} & := \E_{g \sim \cN(\bm{0}_{m_{l-1}},\sigma^2 \I_{m_{l-1}})}\left[ \hat{\vartheta}^{(l)} (\hat{\vartheta}^{(l)})^\top \right] \\
& ~~= \E_{g \sim \cN(\bm{0}_{m_{l-1}},\sigma^2 \I_{m_{l-1}})}\left[ \phi\left( \frac{1}{\sqrt{m_{l-1}}} A^{(l-1)} g\right) \phi \left( \frac{1}{\sqrt{m_{l-1}}} A^{(l-1)} g \right)^\top \1_{[\| \phi ( \frac{1}{\sqrt{m_{l-1}}} A^{(l-1)} g) \|_2 \leq t]} \right] ~. 
\end{align*}
Note that $\lambda_l = \lambda_{\min}(G)$.

By Matrix Chernoff bound, for any $\epsilon \in [0,1)$, we have
\begin{align*}
\P\left( \lambda_{\min}( \hat{A}^{(l)} ( \hat{A}^{(l)})^\top ) \leq (1-\epsilon) \lambda_{\min}( \E_{W_0^{(l)}}[ \hat{A}^{(l)} ( \hat{A}^{(l)})^\top ]) \right) \leq n \left(\frac{e^{-\epsilon}}{(1-\epsilon)^{1-\epsilon}} \right)^{\lambda_{\min}\left(\E_{W_0^{(l)}}[\hat{A}^{(l)} ( \hat{A}^{(l)})^\top ]\right)/t^2}~.
\end{align*}
For $\epsilon=1/2$, with $c_3 = \frac{1}{2}(1 - \log 2)$, we have 
\begin{align*}
\P\left( \lambda_{\min}( \hat{A}^{(l)} ( \hat{A}^{(l)})^\top ) \leq \frac{m_l}{2} \lambda_{\min}(\hat{G}) \right) \leq \exp\left( - \frac{c_3 m_l}{t^2} \lambda_{\min}(\hat{G}) + \log n \right)~,
\end{align*}
where we used the fact that $\E_{W_0^{(l)}}[\hat{A}^{(l)}(\hat{A}^{(l)})^\top]=m_l\E_{g \sim \cN(\bm{0}_{m_{l-1}},\sigma^2 \I_{m_{l-1}})}[\hat{\vartheta}^{(l)}(\hat{\vartheta}^{(l)})^\top]=m_l\hat{G}$. 

With $m_l \geq \frac{t^2}{c_3 \lambda_{\min}(\hat{G})} \log \frac{n}{\bar{\delta}}$, with probability at least $(1-\bar{\delta})$ we have 
\begin{align}
\label{eq:lowerbound_hat_A_l}
\lambda_{\min}( \hat{A}^{(l)} ( \hat{A}^{(l)})^\top ) \geq \frac{m_l}{2} \lambda_{\min}(\hat{G}) ~.
\end{align}
Now, note that
\begin{align*}
\hspace*{-25mm}
\| \hat{G} - G \|_2 & \leq 
 \E_{g \sim \cN(\bm{0}_{m_{l-1}},\sigma^2 \I_{m_{l-1}})} \left\|  \phi\left( \frac{1}{\sqrt{m_{l-1}}} A^{(l-1)} g\right) \phi \left( \frac{1}{\sqrt{m_{l-1}}} A^{(l-1)} g \right)^\top \1_{[\| \phi ( \frac{1}{\sqrt{m_{l-1}}} A^{(l-1)} g) \|_2 \leq t]} \right. \\
 &  \left. \phantom{\E   \phi\left( \frac{1}{\sqrt{m_{l-1}}} A^{(l-1)} g\right) \phi \left( \frac{1}{\sqrt{m_{l-1}}} A^{(l-1)} g \right)^\top } 
 -  \phi\left( \frac{1}{\sqrt{m_{l-1}}} A^{(l-1)} g \right) \phi\left( \frac{1}{\sqrt{m_{l-1}}} A^{(l-1)} g \right)^\top \right\|_2 \\
& = \E_{g \sim \cN(\bm{0}_{m_{l-1}},\sigma^2 \I_{m_{l-1}})}\left[ \left\| \phi \left( \frac{1}{\sqrt{m_{l-1}}} A^{(l-1)} g \right) \right\|_2^2 \1_{[\| \phi ( \frac{1}{\sqrt{m_{l-1}}} A^{(l-1)} g) \|_2 > t]} \right]    \\
& \overset{(a)}{=} \int_{s=0}^{\infty} \P\left( \left\| \phi \left( \frac{1}{\sqrt{m_{l-1}}} A^{(l-1)} g \right) \right\|_2 \1_{[\| \phi ( \frac{1}{\sqrt{m_{l-1}}} A^{(l-1)} g) \|_2 > t]} > \sqrt{s} \right) ds \\
& = \int_{s=0}^{\infty} \P\left( \left\| \phi \left( \frac{1}{\sqrt{m_{l-1}}} A^{(l-1)} g \right) \right\|_2 > t \right) \P\left( \left\| \phi \left( \frac{1}{\sqrt{m_{l-1}}} A^{(l-1)} g \right) \right\|_2 > \sqrt{s} \right) ds \\
& \overset{(b)}{\leq}\exp(2) \exp\left( -c \frac{m_{l-1} t^2 }{2(\sqrt{\log n} +1)^2 \sigma^2 \| A^{(l-1)} \|_F^2} \right) \int_{s=0}^{\infty} \exp\left( -c \frac{m_{l-1} s }{2(\sqrt{\log n} +1)^2 \sigma^2 \| A^{(l-1)} \|_F^2} \right) ds \\
& \overset{(c)}{=} \exp(2) \exp\left( -  \max\left(1 , \log \frac{2a (\sqrt{\log n}  + 1)^2 \sigma^2 \| A^{(l-1)} \|_F^2}{c \lambda_l m_{l-1}} \right)  \right) \frac{2(\sqrt{\log n} +1)^2 \sigma^2 \|A^{(l-1)}\|_F^2}{cm_{l-1}} ~,
\end{align*}
where (a) follows since for any non-negative random variable $Z$,  $\E[Z] = \int_0^{\infty} \P(Z \geq s) ds$, (b) follows from Lemma~\ref{lemm:gammasubg}, and (c) follows from our choice of  $t$ in \eqref{eq:thres} and since for $b > 0$, $\int_0^\infty \exp(-s/b) ds = b$. To simplify further, we consider the following two exhaustive cases:

{\bf Case 1.} Assume
\begin{align*}
\frac{2a(\sqrt{\log n}  + 1)^2 \sigma^2 \| A^{(l-1)} \|_F^2}{c \lambda_l m_{l-1}} \leq \exp(1) \quad \Rightarrow \quad \frac{2 (\sqrt{\log n}  + 1)^2 \sigma^2 \| A^{(l-1)} \|_F^2}{c m_{l-1} }  \leq \frac{\lambda_l}{a} \exp(1)~. 
\end{align*}
Then,
\begin{align*}
\| \hat{G} - G \|_2 & \leq \exp(2) \exp(-1) \frac{2(\sqrt{\log n} +1)^2 \sigma^2 \|A^{(l-1)}\|_F^2}{cm}  \leq \exp(2) \exp(-1) \exp(1) \frac{\lambda_l}{a} = \frac{\exp(2)}{a} \lambda_l \overset{(a)}{\leq} \frac{\lambda_l}{2}~,
\end{align*}
where (a) follows if $a \geq 2 \exp(2)$.

{\bf Case 2.} On the other hand, assume
\begin{align*}
\frac{2a(\sqrt{\log n}  + 1)^2 \sigma^2 \| A^{(l-1)} \|_F^2}{c m_{l-1} \lambda_l} \geq \exp(1) ~. 
\end{align*}
Then,
\begin{align*}
\| \hat{G} - G \|_2 & \leq \exp(2) \frac{c \lambda_l m_{l-1}}{2a (\sqrt{\log n}+1)^2 \sigma^2 \| A^{(l-1)} \|_F^2}  \frac{2(\sqrt{\log n} +1)^2 \sigma^2 \|A^{(l-1)}\|_F^2}{cm_{l-1}} = \frac{\exp(2)}{a} \lambda_l \overset{(a)}{\leq} \frac{\lambda_l}{2}~,
\end{align*}
where (a) follows if $a \geq 2 \exp(2)$. Thus, choosing $a = 15$ in \eqref{eq:thres} ensures $\| \hat{G} - G \|_2 \leq \frac{\lambda_l}{2}$. As a result, 
\begin{equation}
    \label{eq:lowerbound_hat_A_to_A_l}
\lambda_{\min}(\hat{G}) \geq \lambda_{\min}(G) - \|\hat{G} - G \|_2 \geq \lambda_l/2.
\end{equation}
Then, for $m_l \geq \frac{2t^2}{c_3 \lambda_l} \log \frac{n}{\bar{\delta}}$, with probability at least $(1-\bar{\delta})$ we have 
\begin{align*}
\lambda_{\min}(A^{(l)} (A^{(l)})^\top ) & \geq \lambda_{\min}(\hat{A}^{(l)} (\hat{A}^{(l)})^\top ) \overset{(a)}{\geq} \frac{m_l}{2} \lambda_{\min}(\hat{G}) \overset{(b)}{\geq} \frac{m_l}{4} \lambda_l~.
\end{align*}
where (a) follows from~\eqref{eq:lowerbound_hat_A_l} and (b) from~\eqref{eq:lowerbound_hat_A_to_A_l}. Finally, note that we have used $m_l \geq n$ and $m_l \geq \frac{t^2}{c_3 \lambda_{\min}(\hat{G})} \log \frac{n}{\bar{\delta}}$ in the above analysis. Then, with $v = \frac{2 (\sqrt{ \log n} +1)^2 \sigma^2 \| A^{(l-1)} \|_F^2}{c_3 \lambda_l m_{l-1} }$, the choice of $t$ in \eqref{eq:thres}, and $a=15$, and noting that $\lambda_{\min}(\hat{G}) \geq \lambda_l/2$, the analysis holds if we have
\begin{align*}
m_l & \geq \max \left( n,c_2 v \max(1, \log (15 v)) \log \frac{n}{\delta} \right)~.
\end{align*}
for some constant $c_2 > 0$. Choosing $\bar{\delta} = \frac{\delta}{L}$ completes the proof. \qed 




\subsection{Proof of Lemma~\ref{lemm:alphainit1}}
\label{ssec:alphainit}



% We present two versions of a result which establishes $\| \alpha^l(x)\|_2^2 = \Theta(m)$. For the first, we assume the Gaussian variance is $\frac{\sigma_0^2}{c_{\phi,\sigma_0}}$ where $c_{\phi,\sigma_0} := \E_{z \sim \cN(0,\sigma_0^2)}[\phi^2(z)]$. For the second form, we keep the Gaussian variance as $\sigma_0^2$ but used a scaled activation function: $\bar{\phi}(a) = \frac{1}{\sqrt{c_{\phi,\sigma_0}}} \phi(a)$. Both versions yield effectively the same result and are equivalent.  
% \begin{remark}
% \abcomment{update ... their analysis was incorrect} Such scaling has appeared in earlier work with smooth activation functions [Du et al.].
% \end{remark}

% \alphainit*

% \proof We do the proof by induction. For $l=0$, $\| \alpha^{(0)}(x) \|_2^2 = \| x \|_2^2 =  c_{\phi,\sigma_0} d$.  For $l=0$ and $m_0 = d$, so the result is satisfied at $l=0$ almost surely.

% Assume that the result holds for a certain $l$, so that
% \begin{align}
% c_{\phi,\sigma_0} \left(1 -  \frac{h_C(l)}{2h_C(L)}\right) m_l  \leq \| \alpha^l(x) \|_2^2 \leq c_{\phi,\sigma_0} \left(1 +  \frac{h_C(l)}{2h_C(L)}\right) m_l \nonumber  \\
% \Rightarrow \quad - \frac{h_C(l)}{2h_C(L)}  \leq \frac{\| \alpha^l(x) \|_2^2}{c_{\phi,\sigma_0} m_l} - 1 \leq  \frac{h_C(l)}{2h_C(L)} ~.
% \label{eq:rip1}
% \end{align}
% We condition on $\{ W_0^{(l')}, l' \in [l] \}$, and focus on layer $\alpha^{(l+1)}$ with random weights $W_0^{(l+1)} = [w_{1,:}; \cdots;w_{m_{l+1},:}] \in \R^{m_{l+1} \times m_l}$. Note that $\|\alpha^{(l+1)}(x) \|_2^2 = \sum_{j=1}^{m_{l+1}} (\alpha^{(l+1)}_j(x))^2$.  Since $\phi$ is 1-Lipschitz and $\phi(0)=0$, $|\phi(a)| \leq |a|$, we have
% \begin{align}
% \E_{W_0^{(l+1)}}\| \alpha^{(l+1)}(x) \|_2^2 & = \sum_{j=1}^{m_{l+1}} \E_{w_{j,:}} [(\alpha^{(l+1)}_j(x))^2] = m_{l+1} \E_{g \sim \cN\left(0,\frac{\sigma_0^2}{c_{\phi,\sigma_0}} \I\right)}\left[ \phi^2\left(\frac{1}{\sqrt{m_l}}\langle g, \alpha^{(l)}(x) \rangle \right) \right]~\nonumber \\
% & = m_{l+1} \E_{g \sim \cN\left(0,\frac{\sigma_0^2}{c_{\phi,\sigma_0}} \I\right)}\left[ \phi^2\left(\frac{\| \alpha^{(l)}(x)\|_2}{\sqrt{m_l}} \left\langle g, \frac{\alpha^{(l)}(x)}{\| \alpha^{(l)}(x)\|_2} \right\rangle \right) \right] \nonumber \\
% & = m_{l+1}  \E_{z \sim \cN\left(0,\frac{\sigma_0^2}{c_{\phi,\sigma_0}}\right)}\left[ \phi^2\left(\frac{\| \alpha^{(l)}(x)\|_2}{\sqrt{m_l}} z \right) \right] \\
% & = m_{l+1}  \E_{z \sim \cN(0,\sigma_0^2)}\left[ \phi^2\left(\frac{\| \alpha^{(l)}(x)\|_2}{\sqrt{c_{\phi,\sigma_0}m_l}} z \right) \right]
% \label{eq:rip2}
% \end{align}
% From Proposition~\ref{prop:gauss2} with $\beta = \frac{\| \alpha^{(l)}(x)\|_2}{\sqrt{c_{\phi,\sigma_0 m_l}}}$, we have 
% \begin{align}
% c_{\phi,\sigma_0} - \sigma_0^2 \left| \frac{\| \alpha^l(x) \|_2^2}{c_{\phi,\sigma_0} m_l} - 1 \right| & \leq \E_{z \sim \cN(0,\sigma_0^2)}\left[ \phi^2\left(\frac{\| \alpha^{(l)}(x)\|_2}{\sqrt{c_{\phi,\sigma_0}m_l}} z \right) \right] 
%     \leq c_{\phi,\sigma_0} + \sigma_0^2 \left| \frac{\| \alpha^l(x) \|_2^2}{c_{\phi,\sigma_0} m_l} - 1 \right| \nonumber \\
% \overset{(a)}{\Rightarrow} \quad c_{\phi,\sigma_0}\left( 1 - \frac{c_0 h_C(l)}{2h_C(L)} \right) & \leq \E_{z \sim \cN(0,\sigma_0^2)}\left[ \phi^2\left(\frac{\| \alpha^{(l)}(x)\|_2}{\sqrt{c_{\phi,\sigma_0} m_l}} z \right) \right] 
%   \leq c_{\phi,\sigma_0}\left( 1 + \frac{c_0 h_C(l)}{2h_C(L)} \right)~,  
% %\Rightarrow \quad c_{\phi,\sigma_0}\left( 1 - \frac{h_C(l+1)}{2h_C(L)} \right) & \leq \E_{z \sim \cN(0,\sigma_0^2)}\left[ \phi^2\left(\frac{\| \alpha^{(l)}(x)\|_2}{\sqrt{m_l}} z \right) \right]   \leq c_{\phi,\sigma_0}\left( 1 + \frac{h_C(l+1)}{2h_C(L)} \right)~,
%  \label{eq:rip3}
% \end{align}
% where (a) follows from \eqref{eq:rip1}. 
% %and (b) follows by the definition of $h_C(l)$.

% Combining \eqref{eq:rip2} and \eqref{eq:rip3}, we have 
% \begin{align}
% c_{\phi,\sigma_0} \left(1 -  \frac{c_0 h_C(l)}{2h_C(L)}\right) m_{l+1}  \leq \E_{W_0^{(l+1)}}\| \alpha^{(l+1)}(x) \|_2^2 \leq c_{\phi,\sigma_0} \left(1 +  \frac{c_0 h_C(l)}{2h_C(L)}\right) m_{l+1}~.
% \label{eq:rip4}
% \end{align}

% Let $\kappa:= \| (\alpha_j^{(l+1)}(x))^2 \|_{\psi_1}$. Then, from Lemma~\ref{lemm:gammasubg} and \eqref{eq:rip1}, we have
% $\kappa  = \| (\alpha_j^{(l+1)}(x)) \|^2_{\psi_2} \leq \frac{4 \sigma^2}{m_l} \| \alpha^{(l)} \|_2^2 \leq 6 c_{\phi,\sigma_0} \sigma^2 = \tilde{O}(1)$. Conditioned on $\{ W_0^{(l')}, l' \in [l] \}$, since $\alpha_j^{(l+1)}(x), j \in [m_{l+1}]$ are independent, from Bernstein's inequality we have 
% \begin{align*}
% \P\left( \left| \sum_{j=1}^{m_{l+1}} (\alpha_j^{(l+1)}(x))^2 - \E_{W_0^{(l+1)}}\| \alpha^{(l+1)}(x) \|_2^2  \right| \geq t \right) \leq 2 \exp\left[-c \min\left(\frac{t^2}{m_{l+1} \kappa^2} , \frac{t}{\kappa} \right) \right]
% \end{align*}
% Choosing $t = \frac{c_{\phi,\sigma_0}}{2h_C(L)} \frac{\kappa}{\min(c,\sqrt{c})} (m_{l+1})^{3/4} \log m_{l+1} \leq \frac{c_{\phi,\sigma_0}}{2h_C(L)} m_{l+1}$, we have 
% \begin{align*}
% \E_{W_0^{(l+1)}}\| \alpha^{(l+1)}(x) \|_2^2 - \frac{c_{\phi,\sigma_0}}{2h_C(L)} m_{l+1}  & ~\leq~  \| \alpha^{(l+1)}(x) \|_2^2  ~\leq~  E_{W_0^{(l+1)}}\| \alpha^{(l+1)}(x) \|_2^2 + \frac{c_{\phi,\sigma_0}}{2h_C(L)} m_{l+1} \\
% \overset{(a)}{\Rightarrow} \quad  c_{\phi,\sigma_0} \left( 1 - \frac{1 + c_0 h_C(l)}{2h_C(L)} \right) m_{l+1} & ~\leq ~  \| \alpha^{(l+1)}(x) \|_2^2  ~ \leq ~  c_{\phi,\sigma_0} \left( 1 - \frac{1 + c_0 h_C(l)}{2h_C(L)} \right) m_{l+1} \\
% \overset{(b)}{\Rightarrow} \quad c_{\phi,\sigma_0} \left( 1 - \frac{h_C(l+1)}{2h_C(L)} \right) m_{l+1} & ~\leq ~  \| \alpha^{(l+1)}(x) \|_2^2  ~ \leq ~  c_{\phi,\sigma_0} \left( 1 - \frac{h_C(l+1)}{2h_C(L)} \right) m_{l+1}~,
% \end{align*}
% where (a) follows from \eqref{eq:rip4} and (b) follows since $h_C(l+1) = 1 + c_0 h_C(l)$, with probability at least 
% \begin{align*}
% 1 - 2 \exp\left[ - \min \left( \frac{c^2_{\phi,\sigma_0} \sqrt{m_{l+1}}}{8 h_C(L)^2}, \frac{c_{\phi,\sigma_0} \sqrt{m_{l+1}}}{4 h_C(L)}  \right) 2\log m_{l+1}\right] \leq 1 - \frac{2}{m_l}~.
% \end{align*}
% Applying union bound over all layers completes the proof. \qed 

% \abedit{Let $a_0 = c_0^2$. Recall that $L \leq \log n$, we have $h_C(L) = \frac{c_0^L-1}{c_0 - 1} \leq L c_0^L$, so that $h_C^2(L) \leq L^2 (a_0)^L \leq (\log n)^2 a_0^L \leq (\log n)^2 n^{\log a_0}$. Then, it suffices to have $m_{l+1} = \tilde{\Omega}(n^{\log a_0})$ where $a_0 = c_0^2 = \frac{\sigma_0^4}{c_{\phi,\sigma}^2}$. For $\phi(a)=a$, $c_0=a_0=1$, so from this analysis, $\tilde{\Omega}(1)$ width suffices (but linear may break due to other reasons). For ReLU, $c_0 = 2$, so $a_0=4$, and $\tilde{\Omega}(n^{1.39})$ width suffices, for this part of the analysis. For GeLU, $c_0$ will be a bit smaller, so mildly larger width will be needed}
%
% \abcomment{write the above formally ... we have the result!}

\alphainit*

\proof We do the proof by induction. Let $x \in \{x_i, i \in [n]\}$. For $l=0$, $\| \alpha^{(0)}(x_i) \|_2^2 = \| x_i \|_2^2 =  c_{\phi,\sigma_0} d$.  For $l=0$ and $m_0 = d$, so the result is satisfied at $l=0$ almost surely.

Assume that the result holds for a certain $l$, so that for any $i \in [n]$
\begin{align}
c_{\phi,\sigma_0} \left(1 -  \frac{h_C(l)}{2h_C(L)}\right) m_l   \leq \min_{i \in [n]} \| \alpha^l(x) \|_2^2 & \leq \max_{i \in [n]} \| \alpha^{(l)}(x) \|_2^2 \leq c_{\phi,\sigma_0} \left(1 +  \frac{h_C(l)}{2h_C(L)}\right) m_l \nonumber  \\
\Rightarrow \quad \max_{i \in [n]} \left| \frac{\| \alpha^{(l)}(x) \|_2^2}{c_{\phi,\sigma_0} m_l} - 1 \right| & \leq  \frac{h_C(l)}{2h_C(L)} ~.
\label{eq:rip1}
\end{align}
We condition on $\{ W_0^{(l')}, l' \in [l] \}$, and focus on layer $\alpha^{(l+1)}$ with random weights $W_0^{(l+1)} = [w_{1,:}; \cdots;w_{m_{l+1},:}] \in \R^{m_{l+1} \times m_l}$. Note that $\|\alpha^{(l+1)}(x) \|_2^2 = \sum_{j=1}^{m_{l+1}} (\alpha^{(l+1)}_j(x))^2$.  Since $\phi$ is 1-Lipschitz and $\phi(0)=0$, $|\phi(a)| \leq |a|$, we have
\begin{align}
\E_{W_0^{(l+1)}}\| \alpha^{(l+1)}(x) \|_2^2 & = \sum_{j=1}^{m_{l+1}} \E_{w_{0,j,:}} [(\alpha^{(l+1)}_j(x))^2] = m_{l+1} \E_{g \sim \cN\left(\bm{0}_{m_l},\frac{\sigma_0^2}{c_{\phi,\sigma_0}} \I_{m_l}\right)}\left[ \phi^2\left(\frac{1}{\sqrt{m_l}}\langle g, \alpha^{(l)}(x) \rangle \right) \right]~\nonumber \\
& = m_{l+1} \E_{g \sim \cN\left(\bm{0}_{m_l},\frac{\sigma_0^2}{c_{\phi,\sigma_0}} \I_{m_l}\right)}\left[ \phi^2\left(\frac{\| \alpha^{(l)}(x)\|_2}{\sqrt{m_l}} \left\langle g, \frac{\alpha^{(l)}(x)}{\| \alpha^{(l)}(x)\|_2} \right\rangle \right) \right] \nonumber \\
& = m_{l+1}  \E_{z \sim \cN\left(0,\frac{\sigma_0^2}{c_{\phi,\sigma_0}}\right)}\left[ \phi^2\left(\frac{\| \alpha^{(l)}(x)\|_2}{\sqrt{m_l}} z \right) \right] \\
& = m_{l+1}  \E_{z \sim \cN(0,\sigma_0^2)}\left[ \phi^2\left(\frac{\| \alpha^{(l)}(x)\|_2}{\sqrt{c_{\phi,\sigma_0}m_l}} z \right) \right].
\label{eq:rip2}
\end{align}
Now, from Proposition~\ref{prop:gauss2} with $\beta = \frac{\| \alpha^{(l)}(x)\|_2}{\sqrt{c_{\phi,\sigma_0 m_l}}}$, we have 
\begin{align}
c_{\phi,\sigma_0} - \sigma_0^2 \left| \frac{\| \alpha^l(x) \|_2^2}{c_{\phi,\sigma_0} m_l} - 1 \right| & \leq \E_{z \sim \cN(0,\sigma_0^2)}\left[ \phi^2\left(\frac{\| \alpha^{(l)}(x)\|_2}{\sqrt{c_{\phi,\sigma_0}m_l}} z \right) \right] 
    \leq c_{\phi,\sigma_0} + \sigma_0^2 \left| \frac{\| \alpha^l(x) \|_2^2}{c_{\phi,\sigma_0} m_l} - 1 \right| \nonumber \\
\overset{(a)}{\Rightarrow} \quad c_{\phi,\sigma_0}\left( 1 - \frac{\vartheta_0^2 h_C(l)}{2h_C(L)} \right) & \leq \E_{z \sim \cN(0,\sigma_0^2)}\left[ \phi^2\left(\frac{\| \alpha^{(l)}(x)\|_2}{\sqrt{c_{\phi,\sigma_0} m_l}} z \right) \right] 
  \leq c_{\phi,\sigma_0}\left( 1 + \frac{\vartheta_0^2 h_C(l)}{2h_C(L)} \right)~,  
%\Rightarrow \quad c_{\phi,\sigma_0}\left( 1 - \frac{h_C(l+1)}{2h_C(L)} \right) & \leq \E_{z \sim \cN(0,\sigma_0^2)}\left[ \phi^2\left(\frac{\| \alpha^{(l)}(x)\|_2}{\sqrt{m_l}} z \right) \right]   \leq c_{\phi,\sigma_0}\left( 1 + \frac{h_C(l+1)}{2h_C(L)} \right)~,
 \label{eq:rip3}
\end{align}
where (a) follows from \eqref{eq:rip1}. 
%and (b) follows by the definition of $h_C(l)$.

Combining \eqref{eq:rip2} and \eqref{eq:rip3}, we have 
\begin{align}
c_{\phi,\sigma_0} \left(1 -  \frac{\vartheta_0^2 h_C(l)}{2h_C(L)}\right) m_{l+1}  \leq \E_{W_0^{(l+1)}}\| \alpha^{(l+1)}(x) \|_2^2 \leq c_{\phi,\sigma_0} \left(1 +  \frac{\vartheta_0^2 h_C(l)}{2h_C(L)}\right) m_{l+1}~.
\label{eq:rip4}
\end{align}

Let $\kappa:= \| (\alpha_j^{(l+1)}(x))^2 \|_{\psi_1}$. Then, we have
$\kappa  = \| (\alpha_j^{(l+1)}(x)) \|^2_{\psi_2} \overset{(a)}{\leq} \frac{4\bar{c} \sigma_0^2}{m_lc_{\phi,\sigma_0}} \| \alpha^{(l)}(x) \|_2^2 \overset{(b)}{\leq} 6\bar{c}\sigma_0^2 = \tilde{O}(1)$,
where (a) follows from a similar procedure to Lemma~\ref{lemm:gammasubg} where $\bar{c}>0$ is some absolute constant, and (b) follows from~\eqref{eq:rip1}. Conditioned on $\{ W_0^{(l')}, l' \in [L] \}$, since $\alpha_j^{(l+1)}(x)$, $j \in [m_{l+1}]$, are independent, from Bernstein's inequality we have 
\begin{align*}
\P\left( \left| \sum_{j=1}^{m_{l+1}} (\alpha_j^{(l+1)}(x))^2 - \E_{W_0^{(l+1)}}\| \alpha^{(l+1)}(x) \|_2^2  \right| \geq t \right) \leq 2 \exp\left[-c \min\left(\frac{t^2}{m_{l+1} \kappa^2} , \frac{t}{\kappa} \right) \right]
\end{align*}
for some absolute constant $c>0$. Then, by union bound 
\begin{align*}
\P\left( \max_{i \in [n]} ~\left| \sum_{j=1}^{m_{l+1}} (\alpha_j^{(l+1)}(x_i))^2 - \E_{W_0^{(l+1)}}\| \alpha^{(l+1)}(x) \|_2^2  \right| \geq t \right) \leq 2n \exp\left[-c \min\left(\frac{t^2}{m_{l+1} \kappa^2} , \frac{t}{\kappa} \right) \right]
\end{align*}
Choosing $t = \frac{c_{\phi,\sigma_0}}{2h_C(L)} \frac{\kappa}{\min(c,\sqrt{c})} (m_{l+1})^{3/4} (\log m_{l+1} + \log n) \leq \frac{c_{\phi,\sigma_0}}{2h_C(L)} m_{l+1}$, we have 
\begin{align*}
\E_{W_0^{(l+1)}}\| \alpha^{(l+1)}(x) \|_2^2 - \frac{c_{\phi,\sigma_0}}{2h_C(L)} m_{l+1}  & \leq \min_{i \in [n]} \| \alpha^{(l+1)}(x_i) \|_2^2 \leq \max_{i \in [n]} \| \alpha^{(l+1)}(x_i) \|_2^2 \leq  E_{W_0^{(l+1)}}\| \alpha^{(l+1)}(x) \|_2^2 + \frac{c_{\phi,\sigma_0}}{2h_C(L)} m_{l+1} \\
\overset{(a)}{\Rightarrow} \quad  c_{\phi,\sigma_0} \left( 1 - \frac{1 + \vartheta_0^2 h_C(l)}{2h_C(L)} \right) m_{l+1} & \leq \min_{i \in [n]} \| \alpha^{(l+1)}(x_i) \|_2^2 \leq \max_{i \in [n]} \| \alpha^{(l+1)}(x_i) \|_2^2 \leq c_{\phi,\sigma_0} \left( 1 - \frac{1 + \vartheta_0^2 h_C(l)}{2h_C(L)} \right) m_{l+1} \\
\overset{(b)}{\Rightarrow} \quad c_{\phi,\sigma_0} \left( 1 - \frac{h_C(l+1)}{2h_C(L)} \right) m_{l+1} & \leq \min_{i \in [n]} \| \alpha^{(l+1)}(x_i) \|_2^2 \leq \max_{i \in [n]} \| \alpha^{(l+1)}(x_i) \|_2^2 \leq  c_{\phi,\sigma_0} \left( 1 - \frac{h_C(l+1)}{2h_C(L)} \right) m_{l+1}~,
\end{align*}
where (a) follows from \eqref{eq:rip4} and (b) follows since $h_C(l+1) = 1 + \vartheta_0^2 h_C(l)$, with probability at least 
\begin{align*}
1 - 2n \exp\left[ - \min \left( \frac{c^2_{\phi,\sigma_0} m_{l+1}^{1/2}}{8 h_C(L)^2}, \frac{c_{\phi,\sigma_0}m_{l+1}^{3/4}}{4 h_C(L)}  \right) 2(\log m_{l+1}+\log n) \right] \geq 1 - \frac{2}{m_l^2}~.
\end{align*}
%\pccomment{When I was trying to derive the last inequality from the equation above, it seems we need to use the condition $\min \left( \frac{c^2_{\phi,\sigma_0} \pc{m_{l+1}^{3/4}}}{8 h_C(L)^2}, \frac{c_{\phi,\sigma_0}\pc{m_{l+1}^{3/4}}}{4 h_C(L)}  \right)\geq 1$, can this be double checked, please?} \abcomment{the first term inside the $\min$ should be a $m_{l+1}^{1/2}$ (reverted), now look at the (lower bound) condition on $m_{l+1}$ in the statement of the Theorem. Also, take a look at Remark 6.1, which shows the lower bound on $m_l$.}
Applying union bound over all layers completes the proof. \qed 

\begin{prop}
Let $c_{\phi,\sigma_0} := E_{z\sim \cN(0,\sigma_0^2)}[\phi^2(z)]$. Then,
%and $c_0 = \frac{\sigma_0^2}{c_{\phi,\sigma_0}}$. Then, 
\begin{align*}
c_{\phi,\sigma_0} - \sigma_0^2 |\beta^2 -1 | \leq \E_{z \sim \cN(0,\sigma_0^2)}[ \phi^2(\beta z)] \leq c_{\phi,\sigma_0} + \sigma_0^2 |\beta^2 -1| ~.
\end{align*}
\label{prop:gauss2}
\end{prop}
\proof We have 
\begin{align*}
\left| \E_{z\sim \cN(0,\sigma_0^2)} [\phi^2( \beta z)] -  E_{z\sim \cN(0,\sigma_0^2)}[\phi^2(z)] \right| 
& \leq  \E_{z\sim \cN(0,\sigma_0^2)}[|\phi^2 (\beta z) - \phi^2(z)|] \\
& = \E_{z\sim \cN(0,\sigma_0^2)}[|\phi(\beta z) -  \phi(z)| |\phi(\beta z) + \phi(z)|] \\ 
& \overset{(a)}{\leq} |\beta - 1| \E_{z\sim \cN(0,\sigma_0^2)}[| z| (|\phi(\beta z)| + |\phi(z)|)] \\
& \overset{(b)}{\leq} |\beta - 1| \E_{z \sim \cN(0,\sigma_0^2)} [|z| (\beta+1)|z|)] \\
&\leq |\beta^2 - 1| \E_{z \sim \cN(0,\sigma_0^2)} [|z|^2] \\
& = \sigma_0^2 |\beta^2 - 1|  ~,
%& = \frac{1}{c_{\phi}}  |\beta -1| 2\E_{z \sim \cN(0,1)}[\phi^2(z)]~,
\end{align*}
where (a) and (b) follows from the $1$-Lipschitzness of $\phi$. As a result, we have 
\begin{align*}
%c_{\phi}^2 - 2|\beta-1| c_{\phi}  \leq  c_{\phi}  \E_{z\sim \cN(0,1)} [\phi^2( \beta z) ] \leq \c_{\phi}^2 +  2|\beta-1| c_{\phi} \\
%\Righatarrow \quad 
c_{\phi,\sigma_0} - \sigma_0^2 |\beta^2-1| & \leq  \E_{z\sim \cN(0,1)} [\phi^2( \beta z) ] \leq c_{\phi,\sigma_0} +  \sigma_0^2 |\beta^2-1| ~.
% \\
% \Rightarrow \quad c_{\phi,\sigma_0}( 1 - c_0 |\beta^2 -1 |) & \leq \E_{z \sim \cN(0,\sigma_0^2)}[ \phi^2(\beta z)] \leq c_{\phi,\sigma_0}(1 + c_0|\beta^2 -1 |)~.
\end{align*}
This completes the proof. \qed 




\subsection{Proof of Lemma~\ref{lemm:lambdahermite}}
\label{ssec:lambdahermite}

We start with a specific consequence of the Schur product theorem~\cite[Lemma 6.5]{oymak2020hermite} applied to $r$-th order Hadamard product of positive definitive matrices.
\begin{prop}
Let $B = AA^\top$ where $A \in \R^{n \times p}$. Let $b_0 = \min_{i \in [n]} B_{ii}$. Then, for any $r \geq 1$ $\lambda_{\min}( (A A^\top)^{\odot r}) \geq b_0^{r-1} \lambda_{\min}(AA^\top)$.
\label{lemm:schurhad}
\end{prop}
\proof Recall that for PSD matrices $P, Q$, it holds that $\lambda_{\min}(P \odot Q) \geq \min_{i \in [n]} Q_{ii} \cdot \lambda_{\min}(P)$. Further, note that $B_{ii} \geq 0$ and $b_0 \geq 0$ by construction. Further, for any $r \geq 0$, $(B^{\odot r})_{ii} = (B_{ii})^r$. Then,
\begin{align*}
\lambda_{\min}( (A A^\top)^{\odot r}) & = \lambda_{\min}(B^{\odot (r-1)} \odot B) \geq \min_{i \in [n]} (B^{\odot (r-1)})_{ii} \cdot \lambda_{\min}(B)  = b_0^{r-1} \lambda_{\min}(AA^\top)~.
\end{align*}
That completes the proof. \qed 


Now, we are ready to prove Lemma~\ref{lemm:lambdahermite}.

\lambdahermite*

\proof For convenience, let
\begin{align*}
\lambda_{l+1} := \lambda_{\min}\left(  \E_{g \sim 
\cN(\bm{0}_{m_{l}},\sigma^2 \I_{m_{l}})
}\left[ \phi\left( \frac{1}{\sqrt{m_{l}}} A^{(l)} g \right) \phi\left( \frac{1}{\sqrt{m_{l}}} (A^{(l)} g)^\top\right) \right] \right)
\end{align*}
Let $U_l \in \R^{n \times m_l}$ have $i$th row $U_{l,i:} = \frac{\alpha^{(l)}(x_i)}{\|\alpha^{(l)}(x_i)\|_2}$, so that $U_l$ is a row normalized version of $A^{(l)}$. Let $C_l = \diag(c_{l,i})$ where $c_{l,i} = \frac{\|\alpha^{(l)}(x_i)\|_2}{\sqrt{m_l}}$. Note that $\frac{1}{\sqrt{m_l}} A^{(l)} = C_l U_l$. Further, from Lemma~\ref{lemm:alphainit1}, $\min_{i,l} c_{l,i} \geq \sqrt{\frac{c_{\phi,\sigma_0}}{2}}$ and $\max_{i,l} c_{l,i} \leq \sqrt{\frac{3c_{\phi,\sigma_0}}{2}}$ with probability at least $1 - \frac{2L}{m^2}$.
Let $M^{(l)}_r(\phi) = \diag\left( \mu_r^{[c_i^2 \sigma^2]}(\phi) \right)$, and let $(\mu_{r,0}^{(l)})^2 = \min_{i \in [n]} \left( \mu_r^{[c_i^2 \sigma^2]}(\phi) \right)^2$.
Then, for any integer $r > 0$, we have 
\begin{align*}
\lambda_{l+1} & = \lambda_{\min} \left( \E_{g \sim 
\cN(\bm{0}_{m_{l}},\sigma^2 \I_{m_{l}})
}\left[ \phi\left( C_l U_l g\right) \phi\left( C_l U_l g\right)^\top \right] \right) \\
& \overset{(a)}{\geq} \sigma^{6r} \left( \frac{c_{\phi,\sigma_0}}{2} \right)^{3r} \lambda_{\min} \left( (M_r^{(l)}(\phi) (U_l)^{\star r}) (M_r^{(l)}(\phi) (U_l)^{\star r})^\top \right)~\\ 
& \overset{(b)}{\geq} (\mu_{r,0}^{(l)})^2 \sigma^{6r} \left( \frac{c_{\phi,\sigma_0}}{2} \right)^{3r} \lambda_{\min} \left( ((U_l)^{\star r}) ((U_l)^{\star r})^\top \right)~\\ 
& \geq (\mu_{r,0}^{(l)})^2 \sigma^{6r} \left( \frac{c_{\phi,\sigma_0}}{2} \right)^{3r} \lambda_{\min} \left(( U_l U_l^\top)^{\odot r} \right)~\\ 
& \overset{(c)}{\geq} (\mu_{r,0}^{(l)})^2 \sigma^{6r} \left( \frac{c_{\phi,\sigma_0}}{2} \right)^{3r} \lambda_{\min} \left( U_l U_l^\top \right) \\
& = (\mu_{r,0}^{(l)})^2 \sigma^{6r} \left( \frac{c_{\phi,\sigma_0}}{2} \right)^{3r} \frac{1}{m_l}  \lambda_{\min} \left( C_l^{-1} A^{(l)} (A^{(l)})^\top C_l^{-1} \right) \\
& \geq (\mu_{r,0}^{(l)})^2 \sigma^{6r} \left( \frac{c_{\phi,\sigma_0}}{2} \right)^{3r} \frac{2}{3 c_{\phi,\sigma_0}m_l} \lambda_{\min}  \left( A^{(l)} (A^{(l)})^\top \right) \\
& \overset{(d)}{\geq} (\mu_{r,0}^{(l)})^2 \sigma^{6r} \left( \frac{c_{\phi,\sigma_0}}{2} \right)^{3r} \frac{1}{6 c_{\phi,\sigma_0}} \lambda_l~,
\end{align*}
where (a) follows from Lemma~\ref{lemm:hermseries},
\begin{align*}
\E_{\tilde{g} \sim \cN(\bm{0}_{m_l},\sigma^2 \I_{m_l})}\left[ \phi(C_l U_l g) \phi(C_l U_l g)^\top \right] &\succeq \sum_{r'=0}^{\infty}  \sigma^{6r'} (\min_i c_{l,i})^{6r'} (M_r^{(l)}(\phi) (U_l)^{\star r'}) (M_r^{(l)}(\phi) (U_l)^{\star r'})^\top\\
&\succeq 
\sigma^{6r} \left(\frac{c_{\phi,\sigma_0}}{2}\right)^{3r} (M_r^{(l)}(\phi) (U_l)^{\star r}) (M_r^{(l)}(\phi) (U_l)^{\star r})^\top
\end{align*}
for any $r>0$; (b) follows since for a diagonal matrix $M$ with $\mu_0^2 = \min_{i \in [n]} M^2_{ii}$,  
\begin{align*}
\inf_{v : \|v \|_2=1} v^\top (M U) (MU)^\top v & = \inf_{v : \|v \|_2=1} v^\top M (U U^\top) M^\top v \geq \inf_{v : \|v \|_2=1} v^\top M M^\top v  \inf_{w : \|w \|_2=1} w^\top U U^\top w \\
& \geq \mu_0^2 \lambda_{\min}(UU^\top)~;
\end{align*}
(c) follows from Proposition~\ref{lemm:schurhad}; and (d) follows from Lemma~\ref{lemm:highproblambda}.
% Let
% \begin{align*}
% \overline{\lambda}_{l} := \lambda_{\min}\left(  \E_{g \sim \sigma^2 \I_{m_{l}}}\left[ \phi\left( U_{l-1} g \right) \phi\left( U_{l-1} g)^\top\right) \right] \right)
% \end{align*}
% be the normalized version of $\lambda_l$. Then, from Lemma~\ref{lemm:highproblambda}, with probability at least $(1-\frac{\delta}{L})$, we have 
% \begin{align*}
% \lambda_{\min}( U_l U_l^\top ) & \geq \frac{ \overline{\lambda}_l}{4} \\
% & = \frac{1}{4} \lambda_{\min} \left( \E_{g \sim \sigma^2 \I_{m_l}}\left[ \phi\left( U_{l-1} g\right) \phi\left( U_{l-1} g\right)^\top \right] \right) \\
% & \overset{(a)}{\geq} \left( \frac{\mu_r^{[\sigma^2]}(\phi)}{2} \right)^2 \sigma^{6r} \lambda_{\min}(U_{l-1} U_{l-1}^\top)
% \end{align*}
% where (a) follows from Lemma~\ref{lemm:hermseries}. 

Proceeding recursively, using $\sigma^2 = \nu_0^2 = \frac{\sigma_0^2}{c_{\phi,\sigma_0}}$, we have
\begin{align*}
\lambda_{l+1} & \geq\frac{ (\mu_{r,0}^{(l)})^2}{6 c_{\phi,\sigma_0}} \sigma^{6r} \left( \frac{c_{\phi,\sigma_0}}{2} \right)^{3r} \lambda_l \\
& \geq \frac{(\mu_{r,0}^{(l)})^2}{6 c_{\phi,\sigma_0}} \left( \frac{\sigma_0^2}{2} \right)^{3r} \lambda_l \\
& \geq  \left( \frac{(\mu_{r,0}^{(l)})^2}{6 c_{\phi,\sigma_0}} \right)^2 \left( \frac{\sigma_0^2}{2} \right)^{6r} \lambda_{l-1} \\
& \geq \left( \frac{(\mu_{r,0}^{(l)})^2}{6 c_{\phi,\sigma_0}} \right)^l \left( \frac{\sigma_0^2}{2} \right)^{3rl} \lambda_{1} 
% & \geq (\mu_{r,0}^{(l)})^2 \sigma^{6r} \left( \frac{c_{\phi,\sigma_0}}{2} \right)^{3r} \lambda_{\min} \left( U_l U_l^\top \right) \\
% & \geq (\mu_{r,0}^{(l)})^2 \sigma^{6r} \left( \frac{c_{\phi,\sigma_0}}{2} \right)^{3r} \left( \frac{\mu_r^{[\sigma^2]}(\phi)}{2} \right)^2 \sigma^{6r}  \lambda_{\min} \left( U_{l-1} U_{l-1}^\top \right) \\
% & \geq (\mu_{r,0}^{(l)})^2 \left( \frac{\sigma_0^2}{2} \right)^{3r} \sigma^{6rl} \left( \frac{\mu_r^{[\sigma^2]}(\phi)}{2} \right)^{2l} \lambda_{\min}(XX^\top) \\
% & \geq (\mu_{r,0}^{(l)})^2 \left( \frac{\sigma_0^2}{2} \right)^{3r} \left( \frac{\sigma_0^2}{c_{\phi,\sigma_0}} \right)^{3rl} \left( \frac{\mu_r^{[\sigma^2]}(\phi)}{2} \right)^{2l} \lambda_{\min}(XX^\top)~.
\end{align*}
That completes the proof. \qed 


% \begin{align}
% \lambda_{l+1} & \geq \left( \mu_r^{[\sigma^2]}(\phi) \right)^2 \frac{\sigma_0^{6r}c_{\phi,\sigma_0}^{r} m_l^r}{c_{\phi,\sigma_0}^{3r} m_{l}^r} c_{\phi,\sigma_0}^{r-1} m_l^{r-1} \frac{m_l }{4} \lambda_{l} \nonumber \\
% & \geq \frac{\left( \mu_r^{[\sigma^2]}(\phi) \right)^2}{4 c_{\phi,\sigma_0}} \left( \frac{m_l}{\nu_0} \right)^r \lambda_l \nonumber \\
% & \geq \left(\frac{\left( \mu_r^{[\sigma^2]}(\phi) \right)^2}{4 c_{\phi,\sigma_0}} \right)^l \left( \frac{m}{\nu_0} \right)^{rl} \lambda_1~.
% \label{eq:rec1}
% \end{align}
% From Lemma~\ref{lemm:highproblambda}, with probability at least $1- \frac{2L}{m^2}$, using $m_0 =d$ we have 
% \begin{align}
% \lambda_1 & \geq \left( \mu_r^{[\sigma^2]}(\phi) \right)^2 \frac{\sigma^{6r}c_{0}^{2r}}{m_{0}^r} \lambda_{\min}( {A^{(0)}}^{\star r} ({A^{(0)}}^{\star r})^\top  ) \nonumber \\
% & \geq \left( \mu_r^{[\sigma^2]}(\phi) \right)^2 \frac{\sigma_{0}^{6r}c_{\phi,\sigma_0}^{r} m_0^r}{c_{\phi,\sigma_0}^{3r} m_{0}^r} c_{\phi,\sigma_0}^{r-1} m_0^{r-1}\lambda_{\min}( {A^{(0)}} ({A^{(0)}})^\top  ) \nonumber \\
% & = \frac{ \left( \mu_r^{[\sigma^2]}(\phi) \right)^2}{d c_{\phi,\sigma_0}} \left( \frac{d}{\nu_0} \right)^r \lambda_{\min}( X X^\top  )~.
% \label{eq:rec2}
% \end{align}
% Combining \eqref{eq:rec1} and \eqref{eq:rec2}, we have
% \begin{align*}
% \lambda_{l+1} & \geq \left(\frac{\left( \mu_r^{[\sigma^2]}(\phi) \right)^2}{4 c_{\phi,\sigma_0}} \right)^{l+1} \left( \frac{m}{\nu_0} \right)^{rl} \frac{1}{d} \left( \frac{d}{\nu_0} \right)^r \lambda_{\min}( X X^\top  )~.
% \end{align*}
% That completes the proof. \qed

%\abcomment{the lower bound $c_l$ can possibly be obtained from the SubG property of $\alpha_i^{(l)}$ ... variant of Lemma~\ref{lemm:gammasubg}}





\subsection{Background on Hermite Polynomials and Hermite Series Expansions}
\label{ssec:ghermite}
Let $L^2(\R,w(x))$ denote the set of all functions $f : \R \to \R$ such that 
\begin{align}
    \int_{-\infty}^{\infty} f^2(x) w(x) dx < \infty~.
\end{align}
{\bf Probabilist's and Physicist's Hermite Polynomials.} The normalized \emph{probabilist's Hermite  polynomials} are given by:
\begin{align}
H_r(x) = \frac{(-1)^r}{\sqrt{r!}} e^{\frac{x^2}{2}} \frac{d^r}{dx^r} e^{-\frac{x^2}{2}}~.
\label{eq:probherm}
\end{align}
The polynomials are orthogonal with respect to the weight function $w(x) = e^{-\frac{x^2}{2}}$ in the sense that
\begin{align}
\int_{-\infty}^{\infty} H_r(x) H_{r'}(x) w(x) dx & = \sqrt{2\pi} \delta_{r r'}~,
\end{align}
where $\delta_{r r'} = 1$, if $r=r'$, and 0 otherwise, i.e., the Kronecker delta. The corresponding unnormalized probabilist's Hermite polynomials are given by $\bar{H}_r(x) = \sqrt{r!} H_r(x)$. 

The normalized physicist's Hermite polynomials are respectively
\begin{align}
\tilde{H}_r(x) = \frac{(-1)^r}{\sqrt{r!}} e^{x^2} \frac{d^r}{dx^r} e^{-x^2}~.
\label{eq:phyherm}
\end{align}
The polynomials are orthogonal with respect to the weight function $\tilde{w}(x) = e^{-x^2}$ in the sense that
\begin{align}
\int_{-\infty}^{\infty} \tilde{H}_r(x) \tilde{H}_{r'}(x) \tilde{w}(x) dx & = \sqrt{2\pi} 2^r \delta_{r r'}~,
\end{align}
where $\delta_{r r'}$ is the Kronecker delta. The corresponding unnormalized physicist's Hermite polynomials are given by $\bar{\tilde{H}}_r(x) = \sqrt{r!} \tilde{H}_r(x)$. 

{\bf Generalized Hermite Polynomials.} Our analysis of potentially inhomogeneous activation functions will need the substantially more flexible notion of normalized \emph{generalized Hermite polynomials} $H_r^{[a]}(x)$, for a given $a>0$, which are orthogonal with respect to $w^{[a]}(x) = \frac{1}{\sqrt{2\pi a}} e^{-x^2/2a}$, and are given by
\begin{align}
    H_r^{[a]}(x) =  \frac{(-1)^r}{\sqrt{r!}} e^{\frac{x^2}{2a}} \frac{d^r}{dx^r} e^{-\frac{x^2}{2a}}~.
\label{eq:genherm}
\end{align}
It is easy to see that $H_r^{[1]}(x) = H_r(x)$, the probabilist's Hermite polynomial in \eqref{eq:probherm}, and $H_r^{[\frac{1}{2}]} = \tilde{H}_r(x)$, the physicist's Hermite polynomial in \eqref{eq:phyherm}. Furthermore, the generalized Hermite polynomials can be written as scaled versions of probabilist's Hermite polynomials as
\begin{align}
    H_r^{[a]}(x) = a^{\frac{r}{2}} H_r\left( \frac{x}{\sqrt{a}} \right)~.
\label{eq:hermtrans}
\end{align}

{\bf Hermite Series.} The polynomials $\{ H_r(x) \}_{r=0}^{\infty}$ form an orthonormal basis for $L^2\left(\R,\frac{e^{-x^2/2}}{\sqrt{2\pi}}\right)$ which is a Hilbert space with inner product
\begin{align}
\langle \phi_1, \phi_2 \rangle = \int_{-\infty}^{\infty} \phi_1(x) \phi_2(x) \frac{e^{-x^2/2}}{\sqrt{2\pi}} dx ~.
\end{align}
Thus, any function in $L^2\left(\R,\frac{e^{-x^2/2}}{\sqrt{2\pi}}\right)$ can be represented as a Hermite series expansion
\begin{align}
    \phi(x) = \sum_{r=0}^{\infty} \mu_r(\phi) H_r(x) ~,
\end{align}
where $\mu_r(\phi)$ is the $r$-th Hermite coefficient given by
\begin{align}
\mu_r(\phi) = \int_{-\infty}^{\infty} \phi(z) H_r(z) \frac{e^{-z^2/2}}{\sqrt{2\pi}} dz ~.
\end{align}
Note that $\phi \in L^2\left(\R,\frac{e^{-x^2/2}}{\sqrt{2\pi}}\right)$ if and only if $\| \phi \|^2 = \langle \phi,\phi \rangle = \sum_{r=0}^{\infty} \mu_r^2(\phi) < \infty$.

For our analysis with inhomogeneous activation functions, we will need to use Hermite series expansions with generalized Hermite polynomials. The polynomials $\{ H_r^{[a]}(x) \}_{r=0}^{\infty}$ form an orthonormal basis for $L^2\left(\R,\frac{e^{-x^2/2a}}{\sqrt{2\pi a}}\right)$ which is a Hilbert space with inner product
\begin{align}
\langle \phi_1, \phi_2 \rangle = \int_{-\infty}^{\infty} \phi_1(x) \phi_2(x) \frac{e^{-x^2/2a}}{\sqrt{2\pi a}} dx ~.
\end{align}
Any function in $L^2\left(\R,\frac{e^{-x^2/2a}}{\sqrt{2\pi a}}\right)$ can be represented as a Hermite series expansion:
\begin{align}
    \phi(x) = \sum_{r=0}^{\infty} \mu_r^{[a]}(\phi) H_r^{[a]}(x) ~,
\end{align}
where $\mu_r^{[a]}(\phi)$ is the $r$-th Hermite coefficient given by
\begin{align}
\mu_r^{[a]}(\phi) = \int_{-\infty}^{\infty} \phi(z) H_r^{[a]}(z) \frac{e^{-z^2/2a}}{\sqrt{2\pi a}} dz ~.
\end{align}
Note that $\phi \in L^2\left(\R,\frac{e^{-x^2/2a}}{\sqrt{2\pi a}}\right)$ if and only if $\| \phi \|^2 = \langle \phi,\phi \rangle = \sum_{r=0}^{\infty} (\mu_r^{[a]}(\phi))^2 < \infty$.


\subsection{Expectation of Product of Hermite Polynomials}
Our NTK analysis for general activation functions, including inhomogeneous functions, depends on the following key result on expectation of product of Hermite polynomials. The equivalent prior analysis in~\cite{oymak2020hermite,ng2020hermite1,ng2021hermite2} only works for homogeneous functions, and uses basic Hermite polynomials. Our general analysis instead uses generalized Hermite polynomials.

\begin{lemm}
Let $\u_x,\u_y \in \R^d$ be unit vectors, and let $c_x, c_y \in \R_{++}$ be positive constants. Then, for $r,r'=0,1,\ldots$ and $\delta_{rr'}$ denoting the Kronecker delta, we have
\begin{align}
\E_{\tilde{\g} \sim \cN(\bm{0}_d,\sigma^2 \I_d)}\left[ H_r^{[c_x^2 \sigma^2]}(c_x \langle \tilde{\g}, \u_x\rangle) H_{r'}^{[c_y^2 \sigma^2]}(c_y \langle \tilde{\g}, \u_y \rangle) \right] = \sigma^{6r}  c_x^{3r} c_y^{3r} \langle \u_x, \u_y \rangle^r \delta_{rr'}~.
\end{align}
\label{lemm:hermprod}
\end{lemm}
\proof Let $\g \sim \cN(\bm{0},\I_d)$ so that $\sigma\g$ is identically distributed as $\tilde{\g} \sim \cN(\bm{0},\sigma^2 \I_d)$, and consider any $s,t,\in\R$. Then,
\begin{align*}
\E_{\tilde{\g} \sim \cN(\bm{0}_d,\sigma^2 \I_d)}\left[ \exp(s c_x \langle \tilde{\g},\u_x\rangle + t c_y \langle \tilde{\g},\u_y\rangle) \right] 
& = \E_{\g \sim \cN(\bm{0}_d,\I_d)}\left[ \exp(s\sigma c_x \langle \g,\u_x\rangle + t \sigma c_y \langle \g,\u_y\rangle) \right]\\
& = \prod_{j=1}^d \E_{\g \sim \cN(\bm{0}_d,\I_d)}\left[ \exp(s \sigma c_x g_j u_{x,j} + t \sigma c_y g_j u_{y,j}) \right] \\
& = \prod_{j=1}^d \exp\left( \frac{\sigma^2 (s c_x u_{x,j} + t c_y u_{y,j})^2}{2} \right) \\
& = \exp\left( \frac{s^2 \sigma^2 c_x^2}{2} \| \u_x\|_2^2 + \frac{t^2 \sigma^2 c_y}{2} \| \u_y \|_2^2 + st \sigma^2 c_x c_y \langle \u_x, \u_y \rangle \right) ~,
\end{align*}
so that, since $\|\u_x\|_2^2 = \|\u_y \|_2^2 = 1$, we have
\begin{align}
\E_{\g \sim \cN(\bm{0}_d,\I_d)}\left[ \exp\left(s\sigma c_x \langle \g,\u_x\rangle - \frac{s^2\sigma^2 c_x^2}{2}  \right) \exp \left( t \sigma c_y \langle \g,\u_y\rangle - \frac{t^2 \sigma^2 c_y^2}{2}  \right) \right] =  \exp\left( st \sigma^2 c_x c_y \langle \u_x, \u_y \rangle \right) ~.
\label{eq:hermprod1}
\end{align}
We consider the functions $f,h : \R^d \to \R$ defined as
\begin{align}
    f(s) = \exp \left( s\sigma c_x \langle \g,\u_x \rangle - \frac{s^2\sigma^2 c_x^2}{2} \right)~, \qquad h(t) = \exp \left( t\sigma c_y \langle \g,\u_y\rangle - \frac{t^2\sigma^2 c_y^2}{2} \right)~.
\end{align}
Consider the Taylor expansion of $f(s)$ with respect to $f(0)$ given by
\begin{align}
f(s) = \sum_{r=0}^{\infty} f_r(0) \frac{s^r}{\sqrt{r!}}~, \qquad \text{where} \qquad f_r(0) = \frac{1}{\sqrt{r!}} \left. \frac{d^r}{ds^r} e^{s \sigma c_x \langle \g, \u_x \rangle - \frac{s^2\sigma^2 c_x^2}{2}  } \right|_{s=0}~.
\end{align}
With $z = \langle \g, \u_x \rangle$ and $\tilde{z} = \frac{z}{\sigma c_x}$, we have 
\begin{align*}
f_r(0) & = \frac{1}{\sqrt{r!}} \left. \frac{d^r}{ds^r} e^{s \sigma c_x z - \frac{s^2\sigma^2 c_x^2}{2}  } \right|_{s=0}  \\
& = \frac{1}{\sqrt{r!}} \left. e^{\frac{z^2}{2}} \frac{d^r}{d s^r} e^{-\frac{1}{2} (z - s \sigma c_x)^2} \right|_{s=0} \\
& = \frac{1}{\sqrt{r!}} \left. e^{\frac{z^2}{2}} \frac{d^r}{d s^r} e^{-\frac{\sigma^2 c_x^2}{2} \left( \frac{z}{\sigma c_x} - s \right)^2} \right|_{s=0} \\
& = \frac{1}{\sqrt{r!}} \left. e^{\frac{\sigma^2 c_x^2 \tilde{z}^2}{2}} \frac{d^r}{d s^r} e^{-\frac{\sigma^2 c_x^2}{2} ( \tilde{z} - s )^2} \right|_{s=0} \\
& \overset{(a)}{=} \frac{(-1)^r}{\sqrt{r!}} \left. e^{\frac{\sigma^2 c_x^2 \tilde{z}^2}{2}} \frac{d^r}{d {\tilde{z}}^r} e^{-\frac{\sigma^2 c_x^2}{2} ( \tilde{z} - s )^2} \right|_{s=0} \\
& = \frac{(-1)^r}{\sqrt{r!}} e^{\frac{\sigma^2 c_x^2 \tilde{z}^2}{2}} \frac{d^r}{d {\tilde{z}}^r} e^{-\frac{\sigma^2 c_x^2 \tilde{z}^2}{2}}  \\
& \overset{(b)}{=} H^{\left[\frac{1}{\sigma^2 c_x^2}\right]}_r(\tilde{z})~,
\end{align*}
where (a) follows by the transport or advection equation $\frac{d}{ds} \psi(\tilde{z} - s) = (-1) \frac{d}{d \tilde{z}} \psi(\tilde{z}-s)$ and the equality of mixed partial derivatives for any sufficiently smooth function $\psi$, and (b) follows by definition of generalized Hermite polynomials in \eqref{eq:genherm}. Now, note that
\begin{align*}
H^{\left[\frac{1}{\sigma^2 c_x^2}\right]}_r(\tilde{z}) & \overset{(a)}{=} \frac{1}{\sigma^r c_x^r} H_r(\sigma c_x \tilde{z}) \\
& = \frac{1}{\sigma^r c_x^r} H_r(z) \\
& = \frac{1}{\sigma^r c_x^r} H_r\left( \langle \g, \u_x\rangle \right) \\
& = \frac{1}{\sigma^r c_x^r} H_r\left( \frac{c_x}{\sigma c_x} \langle \tilde{\g}, \u_x \rangle \right) \\
& \overset{(b)}{=} \frac{1}{\sigma^{2r} c_x^{r}} H^{[c_x^2\sigma^2]}_r\left(c_x \langle \tilde{\g}, \u_x\rangle \right)~.
\end{align*}
where (a) and (b) follow from~\eqref{eq:hermtrans}. Thus,
\begin{align}
f(s) = \sum_{r=0}^{\infty} f_r(0) \frac{s^r}{\sqrt{r!}}~, \qquad \text{where} \qquad f_r(0) 
%= H^{\left[\frac{1}{\sigma^2 \|\x\|^2}\right]}_r\left( \frac{1}{\sigma \|\x\|_2} \langle \g,\x \rangle \right) 
= \frac{1}{\sigma^{2r} c_x^{2r}} H^{[c_x^2 \sigma^2]}_r\left( c_x \langle \tilde{\g}, \u_x\rangle \right)~.
\end{align}

Similarly, considering the Taylor expansion of $h(t)$ with respect to $h(0)$, we have 
\begin{align}
h(t) = \sum_{r'=0}^{\infty} h_{r'}(0) \frac{t^{r'}}{\sqrt{r'!}}~, \qquad \text{where} \qquad h_{r'}(0) 
%= H^{\left[\frac{1}{c_y^2 \sigma^2}\right]}_r \left( \frac{1}{\sigma \|\y\|_2} \langle \g,\y \rangle \right)
= \frac{1}{\sigma^{2r'} c_y^{2r'}} H^{[c_y^2\sigma^2]}_{r'} \left( c_y \langle \tilde{\g}, \u_y \rangle \right)~.
\end{align}
Then, from \eqref{eq:hermprod1}, we have 
\begin{align*}
\E_{\tilde{\g} \sim \cN(\bm{0}_d,\sigma^2 \I_d)}&\left[ \left( \sum_{r=0}^{\infty} \frac{1}{\sigma^{2r} c_x^{2r}} H^{[c_x^2 \sigma^2]}_r( c_x \langle \tilde{\g}, \u_x\rangle) \frac{s^r}{\sqrt{r!}} \right)  \left( \sum_{r'=0}^{\infty} \frac{1}{\sigma^{2r'} c_y^{2r'}} H^{[c_y^2 \sigma^2]}_{r'}\left( c_y \langle \tilde{\g}, \u_y \rangle \right) \frac{t^{r'}}{\sqrt{r'!}} \right) \right]\\
&=  \sum_{r=0}^{\infty} \frac{\sigma^{2r} c_x^r c_y^r \langle \u_x, \u_y \rangle^r}{r!} s^r t^r~.
\end{align*}
Since the equality holds for arbitrary $s,t \in R$, equating coefficients of  $s^r t^{r'}$ on both sides, we have 
\begin{align}
\E_{\tilde{\g} \sim \cN(\bm{0}_d,\sigma^2 \I_d)}\left[ H_r^{[c_x^2 \sigma^2]}(c_x \langle \tilde{\g}, \u_x\rangle) H_{r'}^{[c_y^2 \sigma^2]}(c_y \langle \tilde{\g}, \u_y \rangle) \right] = \sigma^{6r} c_x^{3r} c_y^{3r} \langle \u_x, \u_y \rangle^r \delta_{rr'}~,
\end{align}
where $\delta_{rr'}$ is the Kronecker delta. That completes the proof. \qed 

The following result is an important consequence of Lemma~\ref{lemm:hermprod}.

\begin{lemm}
Let $\phi$ be an inhomogeneous activation function. Let $\u_x, \u_y\in\R^d$ be unit vectors and $c_x, c_y$ be positive constants. Then,  we have
\begin{align}
\E_{\tilde{\g} \sim \cN(\bm{0}_d,\sigma^2 \I_d)}\left[ \phi(c_x\langle \tilde{\g}, \u_x \rangle) \phi(c_y\langle \tilde{\g}, \u_y \rangle) \right] = \sum_{r=0}^{\infty} \mu_r^{[c_x^2 \sigma^2]}(\phi) \mu_r^{[c_y^2 \sigma^2]}(\phi) \sigma^{6r} c_x^{3r} c_y^{3r}  \langle \u_x, \u_y \rangle^r ~. 
\end{align}
Further, let $U = [\u_1,\cdots,\u_n]^\top \in \R^{n \times m}$ be such that $\| \u_i \|_2 =1, i \in [n]$. Let $C =\diag(c_i)\in\R^{n\times n}, c_i > 0$, and $c_0 = \min_{i \in [n]} c_i > 0$. Let $M_r(\phi) =  \diag\left( \mu_r^{[c_i^2 \sigma^2]}(\phi)\right)$. Then,
\begin{align}
\E_{\tilde{\g} \sim \cN(\bm{0}_d,\sigma^2 \I_d)}\left[ \phi(C U \tilde{\g}) \phi(C U \tilde{\g})^\top \right] \succeq \sum_{r=0}^{\infty}  \sigma^{6r} c_0^{6r} (M_r(\phi) U^{\star r}) (M_r(\phi) U^{\star r})^\top~,
\end{align}
where $U^{\star r} \in \R^{n \times mr}$ is such that the $i$-th row $U^{\star r}_{i,:} = (\u_i^{\otimes r})^\top$, i.e., $r$ times Kronecker product of $\u_i$ with itself.
\label{lemm:hermseries}
\end{lemm}
\proof Consider the generalized Hermite series expansion of $\phi(\cdot)$ in terms of the generalized Hermite functions $H_n^{[\sigma^2]}$:
\begin{align}
\phi(c_x\langle \tilde{\g}, \u_x \rangle) = \sum_{r=0}^{\infty} \mu_r^{[c_x^2 \sigma^2]}(\phi) H_r^{[c_x^2 \sigma^2]}(c_x \langle \tilde{\g}, \u_x \rangle)~.
\end{align}
Then, we have 
\begin{align*}
\E_{\tilde{\g} \sim \cN(\bm{0}_d,\sigma^2 \I_d)}&\left[ \phi(c_x\langle \tilde{\g}, \u_x \rangle) \phi(c_y\langle \tilde{\g}, \u_y \rangle) \right] \\
& = \E_{\tilde{\g} \sim \cN(\bm{0}_d,\sigma^2 \I_d)}\left[ \left( \sum_{r=0}^{\infty} \mu_r^{[c_x^2 \sigma^2]}(\phi) H_r^{[c_x^2 \sigma^2]}(c\langle \tilde{\g}, \u_x \rangle) \right) \left( \sum_{r'=0}^{\infty} \mu_{r'}^{[c_y^2 \sigma^2]}(\phi) H_{r'}^{[c_y^2 \sigma^2]}(c\langle \tilde{\g}, \u_y \rangle) \right) \right] ~\\
& =  \sum_{r,r'=0}^{\infty} \mu_r^{[c_x^2 \sigma^2]}(\phi) \mu_{r'}^{[c_y^2 \sigma^2]}(\phi) \E_{\tilde{\g} \sim \cN(\bm{0}_d,\sigma^2 \I_d)}\left[H_r^{[c_x^2 \sigma^2]}(c_x \langle \tilde{\g}, \u_x \rangle) H_{r'}^{[c_y^2 \sigma^2]}(c_y \langle \tilde{\g}, \u_y \rangle) \right] \\
& \overset{(a)}{=} \sum_{r=0}^{\infty} \mu_r^{[c_x^2 \sigma^2]}(\phi) \mu_r^{[c_y^2 \sigma^2]}(\phi)  \sigma^{6r} c_x^{3r} c_y^{3r} \langle \u_x, \u_y \rangle^r~.
\end{align*}
%\pccomment{So now the exponent of $c$ is $4r$ instead of $2r$, please double check.}\abcomment{the scaling is $c^{2r}$, similar to $a^{2r}$, not $c^{4r}$.} 
where (a) follows from Lemma~\ref{lemm:hermprod}. 

The matrix case result follows by noting that for any $i, j \in [n]$, $c_i^{3r} c_j^{3r} \geq c_0^{6r}$, $\langle \u_i , \u_j \rangle^r = \langle \u_i^{\otimes r}, \u_j^{\otimes r} \rangle$, and $\mu_r^{[c_i^2 \sigma^2]}(\phi)$ form the diagonal elements of $M_r(\phi)$. That completes the proof. \qed 


\subsection{Additional Remarks on $\lambda_1$}
\label{ssec:lambda1}
The main result in Theorem~\ref{theo:ntk0} establishes $\lambda_{\min}( K_{\ntk}(\cdot ;\theta_0) ) \geq c_0 \lambda_1$ where 
\begin{align*}
\lambda_1 = \lambda_{\min}\left(\E_{g \sim 
\cN(\bm{0}_{d},\sigma^2 \I_{d})}\left[ \phi\left(\frac{1}{\sqrt{d}} X g\right) \phi\left(\frac{1}{\sqrt{d}} X g\right)^\top\right]\right)~,
\end{align*}
where $\sigma^2 = \nu_0^2 = \frac{\sigma_0^2}{c_{\phi,\sigma_0}}$.
We made some high level informal remarks on why and when $\lambda_1 > 0$ in Remark~\ref{rem:lambda1}. Such results have been studied in the recent literature~\citep{SD-JL-HL-LW-XZ:19,DZ-YC-DZ-QG:20,YL-YL:18,ZAZ-YL-ZS:19,oymak2020hermite,ng2021hermite2}. We provide additional details on the topic.

Related to assumptions in \cite{SD-JL-HL-LW-XZ:19}, the simplest analysis comes from assuming $\lambda_{\min}(XX^\top) = c_{\phi,\sigma_0} d \lambda_0 > 0$ for some positive constant $\lambda_0$,  where the scaling is simply because $\|x_i\|_2^2 = c_{\phi,\sigma_0} d$. With $\bar{X}:=\frac{1}{\sqrt{d c_{\phi,\sigma_0}}}X$ so that rows of $\bar{X}$ satisfy $\|\bar{x}_i\|_2 = 1$ and $\lambda_{\min}(\bar{X}\bar{X}^\top) = \lambda_0 > 0$.
%Let $U_l \in \R^{n \times m_l}$ have rows $\u_{l,i} = \frac{\alpha^{(l)}(x_i)}{\|\alpha^{(l)}(x_i)\|_2}$, so that $U_l$ is a row normalized version of $A^{(l)}$. 
Let $C_0 = \diag(c_{0,i})$ where $c_{0,i} = \sqrt{c_{\phi,\sigma_0}}$. Note that $\frac{1}{\sqrt{d}} X = C_0 \bar{X}$. 
%Further, from Lemma~\ref{lemm:alphainit1}, $\min_{i,l} c_{l,i} \geq \sqrt{\frac{c_{\phi,\sigma_0}}{2}}$ and $\max_{i,l} c_{l,i} \leq \sqrt{\frac{3c_{\phi,\sigma_0}}{2}}$ with probability at least $1 - \frac{2L}{m^2}$.
Let $M^{(0)}_r(\phi) = \mu_r^{[\sigma_0^2]}(\phi) \diag( 1)$ \pccomment{Is $\diag( 1)$ the same as the identity matrix? If so, we can perhaps use a notation for the identity matrix such as $I$, though we might need to introduce such notation, maybe just here; I don't think we have introduced the notation $\diag(\cdot)$ either.)}, and let $(\mu_{r,0}^{(0)})^2 =  \left( \mu_r^{[\sigma_0^2]}(\phi) \right)^2$. From Lemma~\ref{lemm:hermseries}, for any integer $r > 0$, we have 
\begin{align*}
\lambda_{1} & = \lambda_{\min} \left( \E_{g \sim \cN(\bm{0}_{d},\sigma^2 \I_{d})}\left[ \phi\left( \frac{1}{\sqrt{d}} X g\right) \phi\left( \frac{1}{\sqrt{d}} X g\right)^\top \right] \right) \\
& \geq \sigma^{6r} \left( c_{\phi,\sigma_0} \right)^{3r} \lambda_{\min} \left( (M_r^{(0)}(\phi) (\bar{X})^{\star r}) (M_r^{(0)}(\phi) (\bar{X})^{\star r})^\top \right)~\\ 
& \geq (\mu_{r,0}^{(0)})^2 \sigma^{6r} \left( c_{\phi,\sigma_0} \right)^{3r} \lambda_{\min} \left( (\bar{X})^{\star r}) (\bar{X})^{\star r})^\top \right)~\\ 
& = (\mu_{r,0}^{(l)})^2 \sigma^{6r} \left( c_{\phi,\sigma_0} \right)^{3r} \lambda_{\min} \left( \bar{X} \bar{X}^\top)^{\odot r} \right)~\\ 
& \geq (\mu_{r,0}^{(l)})^2 \sigma^{6r} \left( c_{\phi,\sigma_0} \right)^{3r} \lambda_{\min} \left( \bar{X} \bar{X}^\top \right) \\
& \geq (\mu_{r,0}^{(l)})^2 \sigma^{6r} \left( c_{\phi,\sigma_0} \right)^{3r} \lambda_0~,
\end{align*}
which gives the desired result.


$\lambda_1$ can also be lower bounded by making assumptions on the activation function $\phi$, e.g., the separability and/or the distribution of $x_i$~\cite{YL-YL:18,ZAZ-YL-ZS:19,oymak2020hermite,ng2021hermite2}. For any unit vector $v$, 
\begin{align*}
\lambda_1(v) & := v^\top \E_{g \sim \cN\left(\bm{0}_{d},\frac{\sigma_0^2}{c_{\phi,\sigma_0}}\I_d\right)}[\phi(\sqrt{c_{\phi,\sigma_0}} \bar{X}g) \phi(\sqrt{c_{\phi,\sigma_0}}  \bar{X}g)^\top] v \\
& = v^\top \E_{g \sim \cN(\bm{0}_d,\sigma_0^2\I_d)}[\phi(\bar{X}g) \phi(\bar{X}g)^\top] v \\
& = \E_{g \sim \cN(\bm{0}_d,\sigma_0^2\I_d)}[ \| \phi(\bar{X}g)^\top v \|_2^2]~.
\end{align*}
Note that with $\tilde{g} = \bar{X}g~, $
it suffices to show $\E_{\tilde{g}}[\langle \phi(\tilde{g}), v \rangle^2] = \E_{Z = \langle \phi(\tilde{g}), v \rangle}[Z^2] \geq \chi_0 > 0$, for some uniform positive constant $\chi_0$ since $\lambda_1 = \inf_v \lambda_1(v)$. For any $c > 0$, by Markov's inequality, we have
\begin{align*}
\P( \| \phi(\bar{X}g)^\top v \|_2 \geq c ) & = \P ( \| \phi(\bar{X}g)^\top v \|_2^2 \geq c^2) \leq \frac{ \E[\| \phi(\bar{X}g)^\top v \|_2^2]}{c^2} \\
\Rightarrow \qquad \E[\| \phi(\bar{X}g)^\top v \|_2^2 & \geq c^2 \P( \| \phi(\bar{X}g)^\top v \|_2 \geq c )~.
\end{align*}
Thus, the problem boils down to lower bounding $\P( \| \phi(\bar{X}g)^\top v \|_2 \geq c )$ for a suitable choice of $c$, or, more conveniently $\P( \| \phi(\bar{X}g)^\top v \|_2 \geq c \|v\|_{\infty} )$ and using $\| v \|_{\infty} \geq \frac{1}{\sqrt{n}}$. Proceeding further rigorously needs specific assumptions on the activation $\phi$, as has been done in recent related work~\citep{oymak2020hermite,ZAZ-YL-ZS:19,YL-YL:18}. 

==> arXiv_RSC/sec/arx1_ntk.tex <==

The smallest eigenvalue of the NTK at initialization plays a crucial role including memorization capacity, global convergence of GD, as well as generalization behavior~\citep{SD-JL-HL-LW-XZ:19,CL-LZ-MB:20,ng2021opt,ng2021hermite2,oymak2020hermite,ZJ-MT:19}. For models with constant depth $L=O(1)$, existing results need $m = \widetilde{\Omega}(n^2)$ for NTK at initialization to be positive definite for smooth actiavtions~\citep{SD-JL-HL-LW-XZ:19}. In this section, we present a sharper analysis showing that  effectively linear width, i.e., $m=\widetilde{\Omega}(n)$, suffices for smooth activations to ensure the NTK at initialization is positive definite. Our analysis builds on prior work on Hermite series expansion of activation functions~\citep{oymak2020hermite,ng2020hermite1,ng2021hermite2}, which have been however restricted to multi-layer ReLU networks, using the homogeneity of ReLU activations. Smooth activations are typically inhomogeneous, so we develop a related but new analysis based on {\em generalized} Hermite polynomials which work for multiple layers of inhomogeneous activations, yielding Theorem~\ref{theo:ntk0}. All detailed proofs are in Appendix~\ref{app:arXiv_ntk}.
\begin{restatable}{theo}{theontk}
Assume that $L=O(1)$ and for $l \in [L]$,
%\begin{align*}
$m_{l}  = m = \Omega( n \log n  \log (Ln/\delta))$.  
%\end{align*}
Let $c_{\phi,\sigma_0} := \E_{z \sim \cN(0,\sigma_0^2)}[\phi^2(z)]$ and $\nu_0^2 := \frac{\sigma_0^2}{c_{\phi,\sigma_0}}$. Then, assuming $w^{(l)}_{0,ij} \sim \cN(0,\nu_0^2), l \in [L]$, with probability at least $1- \delta - \frac{4L}{m}$ over the draw of $\{W_0^{(l)}\}_{l\in[L]}$, for a suitable constant $c_0 > 0$ and $\lambda_1 = \lambda_{\min}(\E_{g \sim \cN(\bm{0}_{d},\nu_0^2 \I_{d})
}[ \phi(\frac{1}{\sqrt{d}} X g) \phi(\frac{1}{\sqrt{d}} X g)^\top])$, we have that the minimum eigenvalue of the NTK at initialization satisfies
%\begin{align*}
$\lambda_{\min}( K_{\ntk}(\cdot ;\theta_0) ) \geq c_0 \lambda_1$.
%\end{align*}
\label{theo:ntk0}
\end{restatable}
%
\begin{remark}
Our results extend to the case of general depth $L$ with essentially no changes in the analysis. For general $L$, the width need to be relaxed to $m_{l} =m= \Omega( n h_C^4(L) \log n  \log (n/\delta))$ where $h_C(L) = \sum_{i=1}^L \nu_0^{2i}$. Choosing $L = O(1)$ gives Theorem~\ref{theo:ntk0}, and choosing $L = \log \log n$ also yields $m = \widetilde{\Omega}(n)$. 
More generally, if $\nu_0^2 \leq 1$, $h_C(L) = O(L)$, and the width $m$ has $\text{poly}(L)$ dependence, otherwise an $O(c^{O(L)})$ for some $c > 1$ dependence on $L$, similar to \cite{SD-JL-HL-LW-XZ:19}. \qed 
%Further, choosing $L = \log n$ yields $m_{l} = \Omega( n^2  (\log n)^2  \log (n/\delta))$
\end{remark}
\begin{remark}
There are existing approaches in the literature for lower bounding $\lambda_1$ for specific (including smooth) activation functions, using suitable (separability) assumptions on the input $X$~\cite{oymak2020hermite,DZ-YC-DZ-QG:20,ng2021hermite2,SD-JL-HL-LW-XZ:19}. To get an informal sense of a couple of such techniques, let $\bar{X}:=\frac{1}{\sqrt{d}}X$ so that rows of $\bar{X}$ satisfy $\|\bar{x}_i\|_2 =1$. Then, if $\lambda_{\min}(\bar{X} \bar{X}^T) > 0$, then the proof analysis of Theorem~\ref{theo:ntk0} can be extended to show $\lambda_1 > 0$, e.g., see Appendix~\ref{ssec:lambda1}), also~\cite{SD-JL-HL-LW-XZ:19}. Also, for any unit vector $v$, $\lambda_1(v) := v^\top \E[\phi(\bar{X}g) \phi(\bar{X}g)^\top] v = \E[ \| \phi(\bar{X}g)^\top v \|_2^2]$. Note that with $\tilde{g} = \bar{X}g$, it suffices to show $\E_{\tilde{g}}[\langle \phi(\tilde{g}), v \rangle^2] = \E_{Z = \langle \phi(\tilde{g}), v \rangle}[Z^2] > 0$, which is violated only if $Z=0$ a.s. The argument can be made precise by using $g \sim \nu_0^2 \I_d$, properties of $\phi$, Markov's inequality, and separability in $X$~\cite{SD-JL-HL-LW-XZ:19,oymak2020hermite,ng2021hermite2}. We share additional remarks on $\lambda_1$ in Appendix~\ref{ssec:lambda1}. \qed 
\label{rem:lambda1}
\vspace*{-3mm}
\end{remark}

Let $A^{(l)} \in \R^{n \times m_{l}}$ be such that the rows $A^{(l)}_{i,:} = \alpha^{(l)}(x_i)$, i.e., output of layer $l$ for input $x_i, i\in[n]$. \pcedit{We prove that to lower bound $\lambda_{\min}( K_{\ntk}(\cdot ;\theta_0))$ it suffices to lower bound $\lambda_{\min}( A^{(l)} (A^{(l)})^\top )$ for $l\in[L]$; thus the following Theorem~\ref{theo:mineig} is needed.}
%
\begin{restatable}{theo}{mineig}
Assume that $L=O(1)$ and for $l \in [L]$,
%\begin{align*}
$m_{l}  = m = \Omega( n \log n  \log (Ln/\delta))$.  
%\end{align*}
Let $c_{\phi,\sigma_0} := \E_{z \sim \cN(0,\sigma_0^2)}[\phi^2(z)]$ and $\nu_0^2 := \frac{\sigma_0^2}{c_{\phi,\sigma_0}}$. Then, assuming $w^{(l)}_{0,ij} \sim \cN(0,\nu_0^2), l \in [L]$, with probability at least $1- \delta - \frac{4L}{m}$, uniformly over $l \in [L]$ over the draw of $\{W_0^{(l)}\}_{l\in[L]}$, for any integer $r > 1$ we have
\begin{align*}
\lambda_{\min}( A^{(l)} (A^{(l)})^\top ) \geq c_0^{(l-1,r)} m_l \lambda_1~,
\end{align*}
where $c_0^{(l-1,r)}$ is a positive constant and $\lambda_1 = \lambda_{\min}(\E_{g \sim
\cN(\bm{0}_{d},\sigma^2 \I_{d})
}[ \phi(\frac{1}{\sqrt{d}} X g) \phi(\frac{1}{\sqrt{d}} X g)^\top])$. Let $\mu_r^{[q]}(\phi)$, $q>0$, be the $r$-th generalized Hermite coefficient corresponding to the generalized Hermite series expansion  of $\phi$ w.r.t.~$H_r^{[q]}$. Let $c_{l,i} = \frac{\| \alpha^{(l)}(x_i) \|_2}{\sqrt{m_l}}$ and $(\mu_{r,0}^{(l)})^2 = \min_{i \in [n]} \left( \mu_r^{[c_{l,i}^2 \sigma^2]} (\phi) \right)^2$. Then, for any integer $r > 1, l \in [L]_+ = \{0,1,\ldots,L\}$, 
%\begin{align*}
$c_0^{(l,r)} = \left( \frac{(\mu_{r,0}^{(l)})^2}{6 c_{\phi,\sigma_0}} \right)^l \left( \frac{\sigma_0^2}{2} \right)^{3rl}$.
%\end{align*}
\label{theo:mineig}
\end{restatable}

\begin{remark}
Since they are used in Theorem~\ref{theo:mineig}, we provide a self-contained introduction to Hermite Polynomials and Hermite Series Expansions in Appendix~\ref{ssec:ghermite}.
\end{remark}

\begin{remark}
\label{rem:sigma_0}
Smaller initial variance $\sigma_0^2$, based on $\sigma_1 \leq 1$ has a desirable effect on the Hessian and subsequent RSC analysis in Sections~\ref{sec:arXiv_hessian} and \ref{sec:arXiv_rsc-opt}, e.g., $c_H$ in Theorem~\ref{theo:bound-Hess} stays $\widetilde{O}(\poly(L))$. However $\sigma_1 \leq 1$ implies $\sigma_0^2 \leq \frac{1}{4}$, which may affect (exponentially decrease) the constant $c_0^{(l,r)}$ in Theorem~\ref{theo:mineig} \pcedit{and thus the minimum eigenvalue of the NTK since $c_0=\max_{r>1}c_0^{(L-1,r)}$ in Theorem~\ref{theo:ntk0}}. The subtlety here is that the dependence of $c_0^{(l,r)}$ on $\sigma_0^2$ is complex, involving both $c_{\phi,\sigma_0}$ and Hermite coefficient terms.  The issue is mute for $L=O(1)$, but may present a tradeoff for large $L$. \qed. 
\end{remark}

\begin{remark}
A key unique feature of our result and proof is the use of {\em generalized} Hermite coefficients, instead of standard Hermite coefficients in prior work~\citep{oymak2020hermite,ng2020hermite1,ng2021hermite2}. Since smooth activations are typically inhomogeneous, generalized Hermite coefficients help handle multiple layers of inhomogeneous activations which seem difficult with standard Hermite coefficients. Further, our proof technique, based on Hermite expansions, is different from prior related work on smooth activations~\citep{SD-JL-HL-LW-XZ:19} and leads to a sharper sample dependence. We provide a self-contained gentle exposition to generalized Hermite expansions in Appendix~\ref{ssec:ghermite}. \qed 
\end{remark}

\noindent {\em Proof sketch for Theorem~\ref{theo:mineig}.} There are three key parts to the proof: 
\begin{enumerate}[(a)]
\item  showing that under suitable conditions, the minimum eigenvalue of $A^{(l)} (A^{(l)})^\top$ for a model with width $\tilde{\Omega}(n)$ can be lower bounded by a constant scaled version of the minimum eigenvalue of the expectation $\E[A^{(l)} (A^{(l)})^\top]$, i.e., a matrix concentration result; 
\item establishing suitable upper and lower bounds for $\| \alpha^{(l)}\|_2^2$, in particular $\| \alpha^{(l)}\|_2^2 = \Theta(m_l)$ with high probability, which satisfies conditions for the matrix concentration result in (a) above and also helps lower bounding the minimum eigenvalue of the expectation $\E[A^{(l)} (A^{(l)})^\top]$ in (c) below; and 
\item lower bounding the minimum eigenvalue of the expectation $\E[A^{(l)} (A^{(l)})^\top]$ using generalized Hermite series expansion to handle multiple layers of inhomogenous activations and lower bounds on $\| \alpha^{(l)}\|_2^2$ as in (b) above. 
\end{enumerate}
Next we get into the details of each of these results.

\noindent \textbf{(a) Matrix Concentration.} Note that by construction $A^{(l)} = \phi( \frac{1}{\sqrt{m_{l-1}}} A^{(l-1)} (W_0^{(l)})^\top) \in \R^{n \times m_l}$, where $W_0^{(l)} \in \R^{m_{l} \times m_{l-1}}$, $w_{0,ij}^{(l)} \sim \cN(0,\sigma^2)$. In our setting $\sigma^2 = \nu_0^2 = \frac{\sigma_0^2}{c_{\phi,\sigma_0}}$. Through a matrix concentration bound, the minimum eigenvalue of $A^{l} (A^{l})^\top$ can be lower bounded by that of $\E_{W_0^{(l)}}[A^{(l)} (A^{(l)})^\top]$ with high probability, as shown in Lemma~\ref{lemm:highproblambda}. The proof is in Appendix~\ref{ssec:highprobablambda}.

\begin{restatable}[\textbf{Matrix Concentration}]{lemm}{highproblambda}
Let
\begin{align}
\lambda_l := \lambda_{\min}\left(  \E_{g \sim \cN(\bm{0}_{m_{l-1}},\sigma^2 \I_{m_{l-1}})}
\left[ \phi \left( \frac{1}{\sqrt{m_{l-1}}} A^{(l-1)} g \right) \phi \left( \frac{1}{\sqrt{m_{l-1}}} A^{(l-1)} g \right)^\top \right] \right) ~,
\end{align}
and
%\begin{align}
$m_{l} \geq \max ( n, c_2 v \max\big(1, \log(15 v)\big) \log (Ln/\delta) )$,
%\end{align}
where $v := \frac{2(\sqrt{\log n}+1)^2 \sigma^2 \| A^{(l-1)}\|_F^2}{c_3 \lambda_l m_{l-1}}$, and $c_2, c_3$ are absolute constants. Then, with probability at least $(1-\frac{\delta}{L})$ over the draw of $W^{(l)}_0$, we have 
%\begin{align}
$\lambda_{\min}( A^{(l)} (A^{(l)})^\top ) \geq \frac{m_{l} \lambda_l}{4}$.
%\end{align}
\label{lemm:highproblambda}
\end{restatable}
Then, it suffices to upper bound $\| A^{(l-1)} \|_F^2$ and lower bound $\lambda_l$, for $\sigma^2 = \nu_0^2 = \frac{\sigma_0^2}{c_{\phi,\sigma_0}}$.


\noindent \textbf{(b) Bounding $\|A^{(l)}(\x)\|_2^2$.} To bound the Frobenius norm $\| A^{(l)} \|_F^2$, we focus on bounding the $L_2$ norm of each row of $A^{(l)}$ and show that $\|\alpha^l(\x)\|_2^2 = \Theta(m_l)$. In Lemma~\ref{lemm:alphainit1} below, we show that the bound holds uniformly over the dataset $\{\x_i, i\in [n]\}$ with high probability. The proof is in Section~\ref{ssec:alphainit}.
\begin{restatable}[{\bf Bounding $\| \alpha^{(l)}(\x)\|_2^2$}]{lemm}{alphainit}
Let $\{\alpha^{(l)}(\x_i) \in \R^{m_l}, i \in [n]\}$ be the set of output at layer $l$ at initialization for the set of inputs $\{ \x_i, i \in [n]\}$. Let $c_{\phi, \sigma_0} := \E_{z \sim \cN(0,\sigma_0^2)}[\phi^2(z)]$, $\nu_0^2 := \frac{\sigma_0^2}{c_{\phi,\sigma_0}}$, and $h_C(l) := \sum_{i=0}^l \nu_0^{2i}$. Let the depth $L$ be such that $\max\left(\frac{8h_c^2(L)}{c_{\phi,\sigma_0}^2} , \frac{4 h_c(L)}{c_{\phi,\sigma_0}} \right) \leq \sqrt{m_l}, l \in [L]$. Assuming the elements of $W_0^{(l)}, l \in [L]$ are drawn i.i.d.~from $\cN(0,\nu_0^2)$, with probability at least $1 - 2n\sum^L_{l=1}\frac{1}{m_l^2}$ over the draw of $\{W^{(l')}_0, l'\in [L] \}$, uniformly over $l \in [L]$ and $i \in [n]$, we have 
\begin{align*}
\frac{c_{\phi,\sigma_0}}{2} m_l \leq c_{\phi,\sigma_0}\left(1 -  \frac{h_C(l)}{2h_C(L)}\right) m_l  \leq  \| \alpha^{(l)}(x_i) \|_2^2  \leq c_{\phi,\sigma_0} \left(1 + \frac{h_C(l)}{2h_C(L)}\right) m_l \leq \frac{3 c_{\phi,\sigma_0}}{2} m_l~.
\end{align*}
\label{lemm:alphainit1}
\end{restatable}
As a result, by union bound, with probability at least $(1 - 2n\sum_{l=1}^L\frac{1}{m_l^2}) \geq (1 - 2\sum_{l=1}^L\frac{1}{m_l})$ for $m_l \geq n$,
%
%$(1 - \frac{2nL}{m^2}) \geq (1 - \frac{2L}{m})$ for $m \geq n$,
%
uniformly over $l \in [L]$, we have 
%\begin{align}
$\| A^{(l)} \|_F^2 = \sum_{i=1}^n \| \alpha_i^{(l)}\|_2^2 \leq \frac{3 c_{\phi,\sigma_0}}{2}n m_{l}$.
%\label{eq:frobupper0}
%\end{align}
%\abcomment{for simplicity, assuming $\phi(0) =0$, satisfied by almost all activation functions folks use}
Then, under the assumption $m_l=m$, since $\nu_0^2 = \frac{\sigma_0^2}{c_{\phi,\sigma_0}}$, in Lemma~\ref{lemm:highproblambda}, we have $v \leq c_2 \frac{\sigma_0^2 n \log n}{\lambda_l}$, for some constant $c_2>0$. 
%\pccomment{This bound holds if $\log n\geq 1$, which makes sense since typically $n\geq 3$; I guess we shouldn't care much about this.} 
For $L =O(1)$, $h_C^4(L) = O(1) \leq m_l$. As a result, for $l \in [L]$, it suffices to have
\begin{align}
m_{l} & \geq \max\left( n ~,~ c_2 \frac{\sigma_0^2 n \log n}{\lambda_l} \max\left(1, \log \left( c_3 \frac{\sigma_0^2 n \log n}{\lambda_l} \right) \right) \log \frac{Ln}{\delta}  \right) \overset{(a)}{=} \tilde{\Omega}(n)~,
\end{align}
where (a) holds as long as $\lambda_l = \Omega(1)$, which holds with high probability as we show next.
%Thus, in terms of the dependence on the sample size $n$, $m = \tilde{\Omega}(n)$ suffices.

%\abedit{... this should follow by standard analysis, including our results in Section 3, and Lemma C.1 in [NMM21], although we want to (and should be able to) drop the $-\exp(-\Omega(d))$ term in the 'bad probability' part of their result.}

\noindent {\bf (c) Lower Bounding $\lambda_l$.} Next, we focus on lower bounding $\lambda_l$. 
As shown in Lemma~\ref{lemm:lambdahermite}, $\lambda_l$ can be lower bounded in terms of the minimum eigenvalue of the inner product of matrices  ${A^{(l-1)}}^{\star r}$, whose rows are the row-wise Kronecker products of the rows of $A^{(l-1)}$~\citep{oymak2020hermite,ng2020hermite1,ng2021hermite2}. The proof is in Appendix~\ref{ssec:lambdahermite}, and is based on generalized Hermite series expansions.

%\abcomment{result below needs a bit of work}

\begin{restatable}{lemm}{lambdahermite}
Let $c_{\phi,\sigma_0} := \E_{z \sim cN(0,\sigma_0^2)}[\phi^2(z)]$ and $\nu_0^2 := \frac{\sigma_0^2}{c_{\phi,\sigma_0}}$. Let $\mu_r^{[q]}(\phi), q>0$ be the $r$-th generalized Hermite coefficient corresponding to the generalized Hermite series expansion of $\phi$ w.r.t.~$H_r^{[q]}$. Let $c_{l,i} = \frac{\norm{ \alpha^{(l)}(x_i)}_2}{\sqrt{m_l}}$ and $(\mu_{r,0}^{(l)})^2 = \min_{i \in [n]} \left( \mu_r^{[c_{l,i}^2 \nu_0^2]} (\phi) \right)^2$. For any integer $r > 0$,  with probability at least $1-\frac{4L}{m}$, uniformly over $l \in [L]$ we have
\begin{align*}
\lambda_{\min}\left(  \E_{g \sim \cN(\bm{0}_{m_{l}},\sigma^2 \I_{m_{l}})
}\left[ \phi\left( \frac{1}{\sqrt{m_{l}}} A^{(l)} g \right) \phi\left( \frac{1}{\sqrt{m_{l}}} (A^{(l)} g)^\top\right) \right] \right) 
%& \geq \left( \mu_r^{[\nu_0^2]}(\phi) \right)^2 \frac{\nu_0^{6r}c_{l}^{2r}}{m_{l}^r} \lambda_{\min}( {A^{(l)}}^{\star r} ({A^{(l)}}^{\star r})^\top  ) \\
 & \geq \left( \frac{(\mu_{r,0}^{(l)})^2}{6 c_{\phi,\sigma_0}} \right)^l \left( \frac{\sigma_0^2}{2} \right)^{3rl} \lambda_{1} ~.
\vspace*{-3mm}
\end{align*}
%where $\bar{A}_{l}_{(i,:)} = \| A_{l}_{(i,:)} \|_2 A_{l}_{(i,:)}$. \abcomment{the $\bar{A}$ bit can be simplified based on lower bounds on the row norms}
\label{lemm:lambdahermite}
\end{restatable}
Let $c_0^{(l,r)} = \left( \frac{(\mu_{r,0}^{(l)})^2}{6 c_{\phi,\sigma_0}} \right)^l \left( \frac{\sigma_0^2}{2} \right)^{3rl}$. Then, combining Lemma~\ref{lemm:highproblambda} and Lemma~\ref{lemm:lambdahermite}, with probability at least $1-\delta - \frac{4L}{m}$, we have
%\begin{align*}
$\lambda_{\min}(A^{(l)} (A^{(l)})^\top ) \geq \frac{m_l}{4} \lambda_l \geq c_0^{(l-1,r)} m_l \lambda_1$.
%\end{align*}
That completes the proof. \qed 

\begin{remark}
The proof technique \pcedit{used for Theorem~\ref{theo:mineig}}  is general and quite different from influential prior work on multi-layer feedforward networks with smooth activations~\cite{SD-JL-HL-LW-XZ:19}. The approach works for multiple layers of inhomogeneous smooth activation functions unlike prior work using basic Hermite expansions for homogenous activations especially ReLU~\cite{ng2020hermite1,ng2021hermite2}, and possibly the first use of generalized Hermite polynomials in such context. For the activation function $\phi$, we assume $\phi(0)=0$ for simplicity, which can be relaxed similar to our analysis in Section~\ref{sec:arXiv_hessian}.
\end{remark}

